Do Lessons from Metric Learning Generalize to Image-Caption Retrieval?

The triplet loss with semi-hard negatives has become the de facto choice for image-caption retrieval (ICR) methods that are optimized from scratch. Recent progress in metric learning has given rise to new loss functions that outperform the triplet loss on tasks such as image retrieval and representation learning. We ask whether these findings generalize to the setting of ICR by comparing three loss functions on two ICR methods. We answer this question negatively: the triplet loss with semi-hard negative mining still outperforms newly introduced loss functions from metric learning on the ICR task. To gain a better understanding of these outcomes, we introduce an analysis method to compare loss functions by counting how many samples contribute to the gradient w.r.t. the query representation during optimization. We find that loss functions that result in lower evaluation scores on the ICR task, in general, take too many (non-informative) samples into account when computing a gradient w.r.t. the query representation, which results in sub-optimal performance. The triplet loss with semi-hard negatives is shown to outperform the other loss functions, as it only takes one (hard) negative into account when computing the gradient.

==> sections/old_sections/conclusion-v2.tex <==
% !TEX root =  ../main.tex 

\section{Conclusion}

In this work, we contribute to the question if better evaluation performances for the \ac{ICR} task can be obtained by using different loss function(s) than the de facto standard Triplet loss SH. \mdr{We're setting our readers up for disappointment: we're not moving beyond the de facto standard. Needs different packaging. Perhaps as a reproducibility study, contrasting with \citep{chen2020simple,faghri2018vse++}.}
Our main objective is to increase the performance of \ac{ICR} methods without relying on more training data, compute power, or algorithmic improvements.
We compare three loss functions: 
\begin{enumerate*}[label=(\arabic*)]
	\item The Triplet loss with semi-hard negative mining.
	\item NT-Xent loss \cite{chen2020simple}, the corner stone of the recent progress in the field of self-supervised representation learning, and
	\item SmoothAP \cite{brown2020smooth}, a smooth approximation of the average precision metric. 
\end{enumerate*}
We evaluate the three loss function on two \ac{ICR} baseline methods, VSE++ \cite{faghri2018vse++} and VSRN \cite{li2019vsrn}, using two benchmark datasets, Flickr30k \cite{young2014image} and the MS-COCO \cite{lin2014microsoft}.
We show that the Triplet loss SH still yields the best evaluation performances and that the promising results of the NT-Xent loss \cite{chen2020simple} form the representation learning field and the SmoothAP loss \cite{faghri2018vse++} from the metric learning field do not generalize to the \ac{ICR} task.

To obtain a better understanding of why a certain loss function yields better evaluation performances than others, we derive the gradient of each loss function with respect to the query $\vec{q}$ 
We show that the gradient of each loss function w.r.t. $\vec{q}$, has a form of $\vec{v}_{i} - \vec{v}_{j}$ and that each \mdr{loss} function mainly differs on the number of triplets or negatives candidates that are taken into account when computing the gradient w.r.t. query $\vec{q}$.
For every loss function that we consider, we have introduced a methodology to count the number of samples that contribute to the gradient w.r.t.\ $\vec{q}$.
We find that the main explanation why the Triplet loss SH  yields the best overall evaluation performances is because it only takes one negative candidate into account when computing the gradient w.r.t. $\vec{q}$ and the other function take too many non-informative (or easy) samples into account when computing the gradient. 

\mdr{What are the broader implications?}

\mdr{What are the limitations? Below we have two. State these and then formulate clear future directions to address the limitations. Now things are a bit too wordy.}

\header{Counting contributing samples to the gradient}
In this work, we introduce a methodology to count the number of samples that contribute to the gradient w.r.t. query $\vec{q}$.
For the Triplet loss and the Triplet loss SH, there either is a gradient value or there is not.
The gradient value for the Triplet loss or Triplet loss SH is independent of the value of the hyper-parameter $\alpha$. 
For the NT-Xent loss, \cite{chen2020simple} and theSmoothAP loss \cite{brown2020smooth}, however, the contribution of a sample to the gradient is based on a weight value for each sample.

To still be able to count the number of samples, we define a threshold value to turn this weight value into a binary count for the NT-Xent loss and SmoothAP.
Especially the results for NT-Xent loss suggest that turning this weight value into a binary count, by using a threshold value, might be too simplistic to give a good picture of the number of samples that contribute to the gradient. 

The reason for this is that the NT-Xent loss outperforms the Triplet loss for the VSE++ method on de Flickr30k dataset (Table~\ref{table:f30k} row 1.1. and 1.3) while taking on average more negative samples into account than the Triplet loss (Table~\ref{tab:gradcount_triplet} row 1.1  and Table~\ref{tab:gradcount_ntxent} row 1.3). 
This is in contrast with the general finding that taking more negative samples into account when computing the gradient results in lower evaluation scores.
This suggests that the weight value for each candidate has a stronger effect on the gradient computation than we initially thought.
Future work should incorporate the weight value per candidate in the contributing sample count, to incorporate and explain the effect of this weight value per candidate on gradient computation.

\header{Hyper-parameter selection for each loss function}
In this work, we compare three loss functions for the \ac{ICR} task. 
Each function comes with its own hyper-parameter. $\alpha$ for the Triplet loss and Triplet loss SH, and $\tau$ for SmoothAP and NT-Xent. 
The value for each hyper-parameter in this work is selected by either taking the value
\begin{enumerate*}[label=(\roman*)]
	\item  as it has been proposed in its original work, or 
	\item used for the ICR task.
\end{enumerate*}
We did not optimize each hyper-parameter for \ac{ICR} or for a benchmark dataset specifically. 

For each loss function, its hyper-parameter plays a role in the number of samples that contribute to the gradient w.r.t. $\vec{q}$.  
For the Triplet loss, the bigger the value of $\alpha$ the more triplets will violate the margin constraint and therefore contribute to the gradient.
The temperature value $\tau$ for the NT-Xent loss determines how uniform the weight values for the candidates are distributed. 
By using a high $\tau$ value, each candidate will approximately have the same weight value, regardless of the similarity with the query. 
The $\tau$ value for the SmoothAP function determines the steepness of the sigmoid function. 
With a very high value for $\tau$, the operating region of this sigmoid function is very small, and almost no candidate tuple will contribute to the gradient.

It becomes clear that each hyper-parameter plays its own role in how many samples contribute to the gradient. 
In future work we want to investigate how to use the proposed methodology for counting the contributing w.r.t. query $\vec{q}$ to determine the optimal values for $\alpha$ and $\tau$.
We know that the number of contributing samples should be $\approx  1$. Given this number, we can determine what is the optimal value for $\alpha$ and $\tau$,  for each loss function, in different stages in the training process.
This opposed to choosing (fixed) value or do an extensive hyper-parameter search.

==> sections/old_sections/conclusion.tex <==
% !TEX root =  ../main.tex 

\section{Conclusion}

In this work, we contribute to the question if better evaluation performances for the \ac{ICR} task can be obtained by using different loss function(s) than the de facto standard Triplet loss SH. \mdr{We're setting our readers up for disappointment: we're not moving beyond the de facto standard. Needs different packaging. Perhaps as a reproducibility study, contrasting with \citep{chen2020simple,faghri2018vse++}.}
Our main objective is to increase the performance of \ac{ICR} methods without relying on more training data, compute power, or algorithmic improvements.
We compare three loss functions: 
\begin{enumerate*}[label=(\arabic*)]
	\item The Triplet loss with semi-hard negative mining.
	\item NT-Xent loss \cite{chen2020simple}, the corner stone of the recent progress in the field of self-supervised representation learning, and
	\item SmoothAP \cite{brown2020smooth}, a smooth approximation of the average precision metric. 
\end{enumerate*}
We evaluate the three loss function on two \ac{ICR} baseline methods, VSE++ \cite{faghri2018vse++} and VSRN \cite{li2019vsrn}, using two benchmark datasets, Flickr30k \cite{young2014image} and the MS-COCO \cite{lin2014microsoft}.
We show that the Triplet loss SH still yields the best evaluation performances and that the promising results of the NT-Xent loss \cite{chen2020simple} form the representation learning field and the SmoothAP loss \cite{faghri2018vse++} from the metric learning field do not generalize to the \ac{ICR} task.

To obtain a better understanding of why a certain loss function yields better evaluation performances than others, we derive the gradient of each loss function with respect to the query $\vec{q}$ 
We show that the gradient of each loss function w.r.t. $\vec{q}$, has a form of $\vec{v}_{i} - \vec{v}_{j}$ and that each \mdr{loss} function mainly differs on the number of triplets or negatives candidates that are taken into account when computing the gradient w.r.t. query $\vec{q}$.
For every loss function that we consider, we have introduced a methodology to count the number of samples that contribute to the gradient w.r.t.\ $\vec{q}$.
We find that the main explanation why the Triplet loss SH  yields the best overall evaluation performances is because it only takes one negative candidate into account when computing the gradient w.r.t. $\vec{q}$ and the other function take too many non-informative (or easy) samples into account when computing the gradient. 

\mdr{What are the broader implications?}

\mdr{What are the limitations? Below we have two. State these and then formulate clear future directions to address the limitations. Now things are a bit too wordy.}

\header{Counting contributing samples to the gradient}
In this work, we introduce a methodology to count the number of samples that contribute to the gradient w.r.t. query $\vec{q}$.
For the Triplet loss and the Triplet loss SH, there either is a gradient value or there is not.
The gradient value for the Triplet loss or Triplet loss SH is independent of the value of the hyper-parameter $\alpha$. 
For the NT-Xent loss, \cite{chen2020simple} and theSmoothAP loss \cite{brown2020smooth}, however, the contribution of a sample to the gradient is based on a weight value for each sample.

To still be able to count the number of samples, we define a threshold value to turn this weight value into a binary count for the NT-Xent loss and SmoothAP.
Especially the results for NT-Xent loss suggest that turning this weight value into a binary count, by using a threshold value, might be too simplistic to give a good picture of the number of samples that contribute to the gradient. 

The reason for this is that the NT-Xent loss outperforms the Triplet loss for the VSE++ method on de Flickr30k dataset (Table~\ref{table:f30k} row 1.1. and 1.3) while taking on average more negative samples into account than the Triplet loss (Table~\ref{tab:gradcount_triplet} row 1.1  and Table~\ref{tab:gradcount_ntxent} row 1.3). 
This is in contrast with the general finding that taking more negative samples into account when computing the gradient results in lower evaluation scores.
This suggests that the weight value for each candidate has a stronger effect on the gradient computation than we initially thought.
Future work should incorporate the weight value per candidate in the contributing sample count, to incorporate and explain the effect of this weight value per candidate on gradient computation.

\header{Hyper-parameter selection for each loss function}
In this work, we compare three loss functions for the \ac{ICR} task. 
Each function comes with its own hyper-parameter. $\alpha$ for the Triplet loss and Triplet loss SH, and $\tau$ for SmoothAP and NT-Xent. 
The value for each hyper-parameter in this work is selected by either taking the value
\begin{enumerate*}[label=(\roman*)]
	\item  as it has been proposed in its original work, or 
	\item used for the ICR task.
\end{enumerate*}
We did not optimize each hyper-parameter for \ac{ICR} or for a benchmark dataset specifically. 

For each loss function, its hyper-parameter plays a role in the number of samples that contribute to the gradient w.r.t. $\vec{q}$.  
For the Triplet loss, the bigger the value of $\alpha$ the more triplets will violate the margin constraint and therefore contribute to the gradient.
The temperature value $\tau$ for the NT-Xent loss determines how uniform the weight values for the candidates are distributed. 
By using a high $\tau$ value, each candidate will approximately have the same weight value, regardless of the similarity with the query. 
The $\tau$ value for the SmoothAP function determines the steepness of the sigmoid function. 
With a very high value for $\tau$, the operating region of this sigmoid function is very small, and almost no candidate tuple will contribute to the gradient.

It becomes clear that each hyper-parameter plays its own role in how many samples contribute to the gradient. 
In future work we want to investigate how to use the proposed methodology for counting the contributing w.r.t. query $\vec{q}$ to determine the optimal values for $\alpha$ and $\tau$.
We know that the number of contributing samples should be $\approx  1$. Given this number, we can determine what is the optimal value for $\alpha$ and $\tau$,  for each loss function, in different stages in the training process.
This opposed to choosing (fixed) value or do an extensive hyper-parameter search.

==> sections/old_sections/experimental_setup-v2.tex <==
% !TEX root =  ../main.tex 

\section{Experimental Set-up}

We strive to answer the following question: Can performance of  \ac{ICR} methods be improved by using different loss functions, this independent of the method and/or the training data?
We also want to answer the following question: \textit{What is  the relation between the number of candidates that contribute to the gradient w.r.t.\ query $\vec{q}$, and the final evaluation score at the optimal convergence point for each loss function?}
If can define a relation between the number the number of candidates that contribute to the gradient and the final evaluation score, we can either select the best loss function for the \ac{ICR} task or design new loss functions based on this relation.
Below we describe our experimental setup for answering these questions.

\subsection{Datasets}

We focus on two benchmark datasets for the \ac{ICR} task: the Flickr30k~\cite{young2014image} and MS-COCO~\cite{lin2014microsoft} datasets.
Both datasets come with a training, validation and test split. 
We do not use any additional datasets and/or tasks for pre-training the methods. 
For both datasets, each image comes with five captions, each caption only has one positive image.
The Flickr30k dataset comes with a training set of 30,000 images and a test set of 1,000 images. Similar to \cite{karpathy2015deep}, we use 1,000 images from the training set as the validation set. 
We use the MS-COCO training, validation and test split provided by \citet{karpathy2015deep}, which contains 113,287 training images, 5,000 images for validation, and 5,000 for testing.

\subsection{Encoders and optimization}

\MB{Most can be replaced/removed by refering to the github repo}
We evaluate the loss functions described in Section~\ref{sec:method} using two \ac{ICR} methods: VSE++ \cite{faghri2018vse++} and VSRN \cite{li2019vsrn}.
We use both methods mainly as is, except for a few details. 
VSE++ \cite{faghri2018vse++} and VSRN \cite{li2019vsrn} use the same codebase. 
For the  details of the specific  implementations we refer to \cite{faghri2018vse++} and the implementation\footnote{\url{https://github.com/fartashf/vsepp}} for  VSE++ method and  to \cite{li2019vsrn} and the implementation\footnote{\url{https://github.com/KunpengLi1994/VSRN}} for VSRN.
Most of the optimization and training hyper-parameters are the same for both methods (such as number of training epochs, learning rate, embedding sizes, etc.). 
Each method is trained for 30 epochs. 
We start with a learning rate of 0.002 and after 15 epochs we lower the learning rate to 0.0002. 

For  VSE++, we do not apply additional fine-tuning of the image encoder after 30 epochs. 
Our main goal is to have a fair comparison between methods, datasets, and loss functions, not to have the highest overall evaluation scores.
For VSE++, we use ResNet50 \cite{he2016deep} as image-encoder instead of ResNet152 \cite{he2016deep} or VGG \cite{simonyan2014very}. 
ResNet50 is faster to optimize and the performance differences between ResNet50 and ResNet152 are relatively small.

Besides having an image and caption encoder, the  VSRN method comes with an additional caption decoder, to decode the original input caption from the latent image representation, this to add additional supervision to the optimization process. We removed the additional image-captioning module, so as to exclude performance gains on the retrieval tasks due to the optimization of image-captioning. 
In \cite{li2019vsrn}, the similarity score for a query candidate pair, during test and time, is based on averaging the predicted similarity scores of two trained models. 
We only take the predicted relevance score of one model. 
Therefore, our results are lower than the results published in \cite{faghri2018vse++}. 
The reason for this is that the evaluation score improvements are marginal when using the scores of two models (instead of one) but optimizing the methods takes twice as long. 

We run VSE++ and VSRN in the same Python environment with the  newest PyTorch and Python versions. 
We reproduced the results of \cite{faghri2018vse++, li2019vsrn} to validate that the methods were performing as expected in our environment.
Similar to \cite{faghri2018vse++, li2019vsrn}, to prevent over-fitting, we save the best model during training time based on the recall sum score on the validation set.
The full code, and software requirements will be made available upon acceptance.

\subsubsection{Optimization with SmoothAP}

The default implementations of both VSE++ and VSRN iterate over the captions in the dataset set during training time.   
For each training iteration, we sample $n$ captions with their corresponding image.
This results in a batch size of $|\mathcal{B}|  = 2n$ in terms of the samples that we use. 
Because we have $k=5$ captions per image, each image in the training set is sampled and augmented $k$ times during one training epoch. 
However, for SmoothAP we have to sample all the captions that correspond to a caption at once, due to the fact that SmoothAP optimizes a ranking over the captions.
Therefore, the batch size will be  $|\mathcal{B}| = n(k +  1)$, where $k$ is 5 in our case.
To make the comparison between the loss functions fair, we increase the training epochs $k$ times for SmoothAP.
By doing this, we  enforce  that each image in the dataset is sampled just as often as when we optimize with the Triplet loss (SH) or the NT-Xent loss.
The downside of  this is that each caption is sampled $k$ times instead of once per epoch.  
Some initial experiments showed that this does not impact the training significantly. This means that optimizing a method with SmoothAP does not benefit significantly from the fact that the method is optimized with $k$ times more epochs.
When optimizing SmoothAP, we train for 150 epochs and lower the learning rate after 75 epochs.

\subsection{Loss function hyper-parameters}

Each loss function comes with its own hyper-parameter(s). 
We argue that a loss learning function should work 'out of the box', and that results for a specific method or dataset should not significantly dependent on an extensive hyper-parameter search. 
This is why we use each hyper-parameter either 
\begin{enumerate*}[label=(\arabic*)]
	\item as it has been proposed in its original work, or 
	\item used for the ICR task.
\end{enumerate*}
Similar to \cite{faghri2018vse++, li2019visual}, we use $\alpha = 0.2$ for the Triplet loss and Triplet SH for both datasets.
We use  $\tau=0.1$ for the NT-Xent loss \cite{chen2020simple}. 
\citet{chen2020simple} show that a $\tau$ value of $0.1$ results in the best overall evaluation performance on a self-supervised learning task. 
However, for a small batch size (i.e., $\leq 256$) and a small number of training epochs (i.e., $\leq 300$), $\tau=0.5$ resulted in a better evaluation performances. 
Therefore, we did some initial experiments with $\tau=\{0.01, 0.1, 0.5\}$. We found  no big difference in performances between $\tau  = 0.01$ and  $\tau  = 0.1$.
With $\tau  = 0.5$ the performance dropped significantly.
For SmoothAP we use $\tau = 0.01$ \cite{brown2020smooth}.

\subsection{Evaluation metrics}

Both the \ac{i2t} and \ac{t2i} task are evaluated with the Recall@k metric~\citep{lee2018stacked, li2019vsrn, faghri2018vse++, jia2021scaling, messina2021transformer, diao2021similarity, lee2018stacked, li2019vsrn}.
For the  \ac{t2i} task, we have one positive image per caption. 
Therefore, the Recall@k metric measures if the positive image is present in the top-$k$ of the computed ranking. 
For the \text{i2t} tasks, however, we have multiple captions per image. 
Similar to~\citep{lee2018stacked, li2019vsrn, faghri2018vse++, jia2021scaling, messina2021transformer, diao2021similarity, lee2018stacked, li2019vsrn}, we measure if at least \textit{one} of positive captions is present in the top-$k$ of the ranking. 

For the \ac{i2t} task, the Recall@k metric does not provide a full picture on the quality of the total ranking during evaluation.
The reason for this is that only one of the positive captions per image needs to end-up in the top-$k$ of the ranking to get the full recall score, we don't know what the average position/recall is over for all positive captions. 
For this reason, we also evaluate the \ac{i2t} task with the mean Average Precision (mAP) metric. 

\subsection{Experiments}

We run two main experiments.

\header{Comparisons of loss functions for \ac{ICR}}
We evaluate each loss function we described in Section~\ref{sec:method} given a dataset and method.  
For ease of reference, we refer to each individual evaluation with an experiment number (\#) (see Table~\ref{table:f30k} and~\ref{table:coco}).
To reduce the variance in the results we run each combination of method, loss function, and dataset five times and report the average score and standard deviation.
For each run, we evaluate using the Recall@k metric, with $k  =  \{1,5,10\}$, similar to \cite{faghri2018vse++, li2019vsrn}, for both the \acf{i2t} and \acf{t2i} task.
We also report the sum of all the recall scores (rsum) and the average recall value. 
For the \ac{i2t} task, we also report the mean average precision at $5$ (mAP@5).

\header{Counting contributing samples to the gradient}
To count the number of contributing samples to the gradient w.r.t. $\vec{q}$ for each loss function, we introduce the following experimental setup.
We take the checkpoint of one of the five optimized models based on the highest score on the validation set.
We refer to this checkpoint as \textit{the optimal convergence point} for this loss function.
This is not the point with the lowest loss value, but the model checkpoint that results in the highest evaluation scores on the validation set.
We freeze all model parameters and do not apply dropout.

We iterate over the entire training set by sampling random batches $\mathcal{B}$.
For each batch we compute the counts and weight values we defined in Section~\ref{sec:gradcount}. 
We report the mean value and standard deviation over the entire training set.
We do this for both VSE++ and VSRN, for both datasets and each loss function. 
The only hyper-parameter for this experiment is $\epsilon$.
We use a  value of $0.01$ for epsilon for both the NT-Xent and SmoothAP loss.


==> sections/old_sections/experimental_setup.tex <==
% !TEX root =  ../main.tex 

\section{Experimental Set-up}

We strive to answer the following question: Can performance of  \ac{ICR} methods be improved by using different loss functions, this independent of the method and/or the training data?
We also want to answer the following question: \textit{What is  the relation between the number of candidates that contribute to the gradient w.r.t.\ query $\vec{q}$, and the final evaluation score at the optimal convergence point for each loss function?}
If can define a relation between the number the number of candidates that contribute to the gradient and the final evaluation score, we can either select the best loss function for the \ac{ICR} task or design new loss functions based on this relation.
Below we describe our experimental setup for answering these questions.

\subsection{Datasets}

We focus on two benchmark datasets for the \ac{ICR} task: the Flickr30k~\cite{young2014image} and MS-COCO~\cite{lin2014microsoft} datasets.
Both datasets come with a training, validation and test split. 
We do not use any additional datasets and/or tasks for pre-training the methods. 
For both datasets, each image comes with five captions, each caption only has one positive image.
The Flickr30k dataset comes with a training set of 30,000 images and a test set of 1,000 images. Similar to \cite{karpathy2015deep}, we use 1,000 images from the training set as the validation set. 
We use the MS-COCO training, validation and test split provided by \citet{karpathy2015deep}, which contains 113,287 training images, 5,000 images for validation, and 5,000 for testing.

\subsection{Encoders and optimization}

\MB{Most can be replaced/removed by refering to the github repo}
We evaluate the loss functions described in Section~\ref{sec:method} using two \ac{ICR} methods: VSE++ \cite{faghri2018vse++} and VSRN \cite{li2019vsrn}.
We use both methods mainly as is, except for a few details. 
VSE++ \cite{faghri2018vse++} and VSRN \cite{li2019vsrn} use the same codebase. 
For the  details of the specific  implementations we refer to \cite{faghri2018vse++} and the implementation\footnote{\url{https://github.com/fartashf/vsepp}} for  VSE++ method and  to \cite{li2019vsrn} and the implementation\footnote{\url{https://github.com/KunpengLi1994/VSRN}} for VSRN.
Most of the optimization and training hyper-parameters are the same for both methods (such as number of training epochs, learning rate, embedding sizes, etc.). 
Each method is trained for 30 epochs. 
We start with a learning rate of 0.002 and after 15 epochs we lower the learning rate to 0.0002. 

For  VSE++, we do not apply additional fine-tuning of the image encoder after 30 epochs. 
Our main goal is to have a fair comparison between methods, datasets, and loss functions, not to have the highest overall evaluation scores.
For VSE++, we use ResNet50 \cite{he2016deep} as image-encoder instead of ResNet152 \cite{he2016deep} or VGG \cite{simonyan2014very}. 
ResNet50 is faster to optimize and the performance differences between ResNet50 and ResNet152 are relatively small.

Besides having an image and caption encoder, the  VSRN method comes with an additional caption decoder, to decode the original input caption from the latent image representation, this to add additional supervision to the optimization process. We removed the additional image-captioning module, so as to exclude performance gains on the retrieval tasks due to the optimization of image-captioning. 
In \cite{li2019vsrn}, the similarity score for a query candidate pair, during test and time, is based on averaging the predicted similarity scores of two trained models. 
We only take the predicted relevance score of one model. 
Therefore, our results are lower than the results published in \cite{faghri2018vse++}. 
The reason for this is that the evaluation score improvements are marginal when using the scores of two models (instead of one) but optimizing the methods takes twice as long. 

We run VSE++ and VSRN in the same Python environment with the  newest PyTorch and Python versions. 
We reproduced the results of \cite{faghri2018vse++, li2019vsrn} to validate that the methods were performing as expected in our environment.
Similar to \cite{faghri2018vse++, li2019vsrn}, to prevent over-fitting, we save the best model during training time based on the recall sum score on the validation set.
The full code, and software requirements will be made available upon acceptance.

\subsubsection{Optimization with SmoothAP}

The default implementations of both VSE++ and VSRN iterate over the captions in the dataset set during training time.   
For each training iteration, we sample $n$ captions with their corresponding image.
This results in a batch size of $|\mathcal{B}|  = 2n$ in terms of the samples that we use. 
Because we have $k=5$ captions per image, each image in the training set is sampled and augmented $k$ times during one training epoch. 
However, for SmoothAP we have to sample all the captions that correspond to a caption at once, due to the fact that SmoothAP optimizes a ranking over the captions.
Therefore, the batch size will be  $|\mathcal{B}| = n(k +  1)$, where $k$ is 5 in our case.
To make the comparison between the loss functions fair, we increase the training epochs $k$ times for SmoothAP.
By doing this, we  enforce  that each image in the dataset is sampled just as often as when we optimize with the Triplet loss (SH) or the NT-Xent loss.
The downside of  this is that each caption is sampled $k$ times instead of once per epoch.  
Some initial experiments showed that this does not impact the training significantly. This means that optimizing a method with SmoothAP does not benefit significantly from the fact that the method is optimized with $k$ times more epochs.
When optimizing SmoothAP, we train for 150 epochs and lower the learning rate after 75 epochs.

\subsection{Loss function hyper-parameters}

Each loss function comes with its own hyper-parameter(s). 
We argue that a loss learning function should work 'out of the box', and that results for a specific method or dataset should not significantly dependent on an extensive hyper-parameter search. 
This is why we use each hyper-parameter either 
\begin{enumerate*}[label=(\arabic*)]
	\item as it has been proposed in its original work, or 
	\item used for the ICR task.
\end{enumerate*}
Similar to \cite{faghri2018vse++, li2019visual}, we use $\alpha = 0.2$ for the Triplet loss and Triplet SH for both datasets.
We use  $\tau=0.1$ for the NT-Xent loss \cite{chen2020simple}. 
\citet{chen2020simple} show that a $\tau$ value of $0.1$ results in the best overall evaluation performance on a self-supervised learning task. 
However, for a small batch size (i.e., $\leq 256$) and a small number of training epochs (i.e., $\leq 300$), $\tau=0.5$ resulted in a better evaluation performances. 
Therefore, we did some initial experiments with $\tau=\{0.01, 0.1, 0.5\}$. We found  no big difference in performances between $\tau  = 0.01$ and  $\tau  = 0.1$.
With $\tau  = 0.5$ the performance dropped significantly.
For SmoothAP we use $\tau = 0.01$ \cite{brown2020smooth}.

\subsection{Evaluation metrics}

Both the \ac{i2t} and \ac{t2i} task are evaluated with the Recall@k metric~\citep{lee2018stacked, li2019vsrn, faghri2018vse++, jia2021scaling, messina2021transformer, diao2021similarity, lee2018stacked, li2019vsrn}.
For the  \ac{t2i} task, we have one positive image per caption. 
Therefore, the Recall@k metric measures if the positive image is present in the top-$k$ of the computed ranking. 
For the \text{i2t} tasks, however, we have multiple captions per image. 
Similar to~\citep{lee2018stacked, li2019vsrn, faghri2018vse++, jia2021scaling, messina2021transformer, diao2021similarity, lee2018stacked, li2019vsrn}, we measure if at least \textit{one} of positive captions is present in the top-$k$ of the ranking. 

For the \ac{i2t} task, the Recall@k metric does not provide a full picture on the quality of the total ranking during evaluation.
The reason for this is that only one of the positive captions per image needs to end-up in the top-$k$ of the ranking to get the full recall score, we don't know what the average position/recall is over for all positive captions. 
For this reason, we also evaluate the \ac{i2t} task with the mean Average Precision (mAP) metric. 

\subsection{Experiments}

We run two main experiments.

\header{Comparisons of loss functions for \ac{ICR}}
We evaluate each loss function we described in Section~\ref{sec:method} given a dataset and method.  
For ease of reference, we refer to each individual evaluation with an experiment number (\#) (see Table~\ref{table:f30k} and~\ref{table:coco}).
To reduce the variance in the results we run each combination of method, loss function, and dataset five times and report the average score and standard deviation.
For each run, we evaluate using the Recall@k metric, with $k  =  \{1,5,10\}$, similar to \cite{faghri2018vse++, li2019vsrn}, for both the \acf{i2t} and \acf{t2i} task.
We also report the sum of all the recall scores (rsum) and the average recall value. 
For the \ac{i2t} task, we also report the mean average precision at $5$ (mAP@5).

\header{Counting contributing samples to the gradient}
To count the number of contributing samples to the gradient w.r.t. $\vec{q}$ for each loss function, we introduce the following experimental setup.
We take the checkpoint of one of the five optimized models based on the highest score on the validation set.
We refer to this checkpoint as \textit{the optimal convergence point} for this loss function.
This is not the point with the lowest loss value, but the model checkpoint that results in the highest evaluation scores on the validation set.
We freeze all model parameters and do not apply dropout.

We iterate over the entire training set by sampling random batches $\mathcal{B}$.
For each batch we compute the counts and weight values we defined in Section~\ref{sec:gradcount}. 
We report the mean value and standard deviation over the entire training set.
We do this for both VSE++ and VSRN, for both datasets and each loss function. 
The only hyper-parameter for this experiment is $\epsilon$.
We use a  value of $0.01$ for epsilon for both the NT-Xent and SmoothAP loss.


==> sections/old_sections/introduction.tex <==
% !TEX root =  ../main.tex 

\section{Introduction}
\label{section:intro}

\shrink
Given a query item in a particular modality, \emph{cross-modal retrieval} is the task of retrieving similar items in another modality~\cite{zeng2020deep}. 
We focus on \acfi{ICR}~\citep{li2019visual, diao2021similarity, lee2018stacked}. 
For the \ac{ICR} task, given an image or a caption as a query, systems have to retrieve the positive (e.g., matching or similar) item(s) in the other modality.

Most existing \ac{ICR} methods work with a separate encoder for each modality to map the input data to a representation in a shared latent space~\citep{diao2021similarity, li2019vsrn, faghri2018vse++, jia2021scaling, lee2018stacked}. 
The encoders are optimized by using a contrastive-loss criterion, so as to enforce a high degree of similarity between the representations of matching items in the shared latent space.
When performing retrieval using an \ac{ICR} method, a similarity score between a query and each candidate in a candidate set is computed to produce a ranking with the top-$k$ best matching items. 
%The Recall@k measure is the standard evaluation measure for the \ac{ICR} task~\citep{lee2018stacked, li2019vsrn, faghri2018vse++, jia2021scaling, messina2021transformer, diao2021similarity, lee2018stacked}.

A lot of recent work on \ac{ICR} relies on 
\begin{enumerate*}[label=(\arabic*)]
	\item pre-training on large amounts of data \cite{jia2021scaling, radford2021learning, li2020oscar}, and 
	\item more sophisticated (and data-hungry) model architectures \cite{messina2021transformer, faghri2018vse++, li2019vsrn, diao2021similarity, lee2018stacked, chen2020intriguing}.
\end{enumerate*}
However, pre-training at scale on large dataset is not always an option when working on new methods, either due to a lack of the required compute power, or a lack of the data itself, or both.  
For this reason, it is important to develop effective \ac{ICR} methods that only rely on a modest amount of data.

To learn the similarity between the query and the candidates, most \ac{ICR} work relies on the standard Triplet loss with semi-hard negatives~\citep{faghri2018vse++,  li2019vsrn, messina2021transformer, diao2021similarity, lee2018stacked, chen2020intriguing, chen2020imram} or more recently the cross-entropy based NT-Xent~\citep{chen2020simple, chen2020adaptive, jia2021scaling,oord2018representation, gutmann2010noise}) loss.
In \emph{metric learning}, the focus is on loss functions that result in more accurate item representations (in terms of a given evaluation metric) that can distinguish between similar and dissimilar items in a low-dimensional latent space~\citep{musgrave2020metric}.
Most metric learning functions work just with general representations of similar/dissimilar candidates and, in principle, there is no clear argument why obtained results on a specific task/method should not generalize to other modalities and/or domains.
Recent years have witnessed considerable progress in metric learning, with the introduction of new loss functions that result in better evaluation scores on a specific task.  
\mdr{In particular, mention SmoothAP and the benefits that it has brought in metric learning.}
\textit{Can these metric learning approaches, that is, alternative loss functions, be used to increase the performance of \ac{ICR} methods}? 
We compare three different loss function for the \ac{ICR} task: 
\begin{enumerate*}[label=(\arabic*)]
\item the Triplet loss \cite{kiros2014unifying}, including semi-hard negative mining, 
\item NT-Xent loss~\cite{chen2020simple},  and
\item SmoothAP~\cite{brown2020smooth}.
\end{enumerate*}
\mdr{Say something like, ``In the context of metric learning [for which task?], SmoothAP is the winner''}
We experimentally evaluate these three loss functions on fixed methods, with different datasets and with a fixed training regime (i.e. training hyper-parameters) to verify which loss function uses the given training data as effectively as possible.

\if0
\mdr{The following is way too detailed for the introduction.}
This selection of loss functions we use in this work is motivated as follows:
\begin{enumerate}[label=(\arabic*),nosep]
	\item \textbf{NT-Xent}: The Triplet loss with semi-hard negative mining has been the de facto choice as loss function for many \ac{ICR} methods. Recently, some methods \cite{jia2021scaling, chen2020adaptive} have started to use the NT-Xent loss \cite{chen2020simple}. The NT-Xent loss is the cornerstone of the recent progress in the representation learning field, outperforms the Triplet loss with semi-hard negative mining on representation learning tasks \cite{chen2020simple}, and has shown impressive results on multi-modal tasks as well \cite{radford2021learning, jia2021scaling}. However, this has been done in combination with different model architectures and (pre-)training regimes as well. Therefore, it is unclear what the effect is of this alternative loss function is w.r.t.\ the evaluation performance for \ac{ICR} and if it really is a better performing function than the Triplet loss with semi-hard negative mining for the \ac{ICR} task.
	\item \textbf{SmoothAP}: As pointed out above, the down-stream evaluation measure used in the \ac{ICR} task is Recall@k. 
	The Triplet loss and the NT-Xent loss optimize the similarity score between positive and negative candidates in the training batch. However, these loss functions do not give an direct indication of the downstream performance on an evaluation metric, such as Recall@k. The main reason that evaluation metrics are not used as an loss function directly is that most evaluation metrics in information retrieval are discrete (i.e. non-differentiable) and therefore not optimizable with stochastic gradient descent.
	Lately, to overcome this problem, continuous (i.e. smooth) approximations of discrete IR metrics have been introduced. 
	Take, for example, the SmoothAP \cite{brown2020smooth} loss function which is a smooth approximation of the average precision metric. SmoothAP outperforms the Triplet loss on image-to-image retrieval benchmarks \cite{brown2020smooth}, has been successfully applied in representation learning tasks \cite{varamesh2020self}, and does not mainly focus on the mining/weighting of (hard) negatives like most metric learning functions. We want to examine if other loss functions from the metric learning field, which is a approximation of ranking evaluation metric, results in better Recall@k scores, compared to a pair-wise-loss similarity loss like the Triplet loss or NT-Xent loss.
\end{enumerate}
\fi
\if0
\mdr{This sounds too apologetic}
Our goal with this work is not to find the optimal loss function for \ac{ICR} among all possible candidates, but rather to see if promising results from the metric learning field generalize to another domain/task like  \ac{ICR}.
This to encourage 
\begin{enumerate*}[label=(\arabic*)]
	\item the use (or further exploration of) different loss function for \ac{ICR}, to obtain better evaluation performances without requiring different model architectures or extra train data, and
	\item new work on loss function for \ac{ICR} specifically by gaining insights on how different loss functions work for the \ac{ICR} task.
\end{enumerate*}
\fi
Somewhat surprisingly, we find that the lessons from metric learning do not generalize to the \ac{ICR} task: \mdr{One line sumary of main outcomes of contrast experiments.}
To get a better grasp of this unexpected outcome, we propose \AnalysisMethodLong{} (\AnalysisMethod{}), a method for analyzing contrastive loss functions.
%We start with some general prior analyses  \cite{chen2020simple, khosla2020supervised} on the form of the gradients of the Triplet-loss and the NT-Xent loss criteria w.r.t.\ the query and also apply this for the SmoothAP loss function.  
We show that the gradient w.r.t.\ the query for the Triplet loss, NT-Xent and SmoothAP can be formulated as a sum over the representations of the positive and negative candidates in the training batch. The main difference between the three loss functions lies in the number of samples that are used when computing the gradient w.r.t.\ the query.
Using this gradient analysis of each of the loss functions we define a new way of empirically comparing loss functions by counting how many samples contribute to the gradient w.r.t.\ the query representation at the convergence point of the method, which yields an explanation why one loss function outperforms another on the \ac{ICR} task.

\if0
\mdr{Too detailed for the introduction}
We focus on two baseline \ac{ICR} methods, VSE++ \citep{faghri2018vse++} and VSRN~\citep{li2019visual}. 
We have selected these methods because VSRN shares a large part of the VSE++ code base and some of their model architecture (i.e. which is beneficial from a reproducibility point of view). 
For this reason it is easier to compare the methods in a fair manner.
\fi
In summary, we make the following contributions in this paper:
\begin{enumerate}[label=(\arabic*),nosep]
	\item We experimentally compare three loss functions from the metric learning domain to question if promising results from the metric learning field generalize to the \ac{ICR} task, and find that \mdr{wat is de uitkomst}
	\item We propose \AnalysisMethod{}, a new way of analyzing contrastive loss functions, by defining a count that tells us how many candidates in the batch contribute to the gradient w.r.t.\ the query, and \mdr{wat vertelt \AnalysisMethod{} ons over the loss functions?}.
\end{enumerate}



==> sections/old_sections/method/grad_count.tex <==
% !TEX root =  ../../main.tex 

\subsection{Counting contributing samples to the gradient}\label{sec:gradcount}
In paragraph~\ref{par:gradtriplet}, \ref{par:gradntxent} and~\ref{par:gradsmooth}, we have provided the form of the derivative of each loss function w.r.t.\ query $\vec{q}$. Clearly, for each function the derivative is of the form $\vec{v}^{+} - \vec{v}^{-}$. However, each function weights the positive and negative candidate(s) differently and also the number of candidates or triplets that are weighted differs per function. 

In this section we provide, for every loss function that we consider, a methodology to count the number of candidates that contribute to the gradient w.r.t.\ $\vec{q}$. 
The intuition for this is the following: If we compare the gradient w.r.t. $\vec{q}$ for the Triplet loss and the Triplet loss SH, the only difference is the number of triplets that the two loss functions take into account. If two models are optimized in the exact same manner, except one model uses the Triplet loss and the other Triplet loss SH, the difference in performance can only be explained by the fact that Triplet loss sums over all violating triplets and the Triplet loss SH only considers the most violating triplet per query. This means that the number of triplets (i.e. candidates) that contribute to the gradient directly relates to the evaluation performance of the model. The same reasoning applies for the NT-Xent and the SmoothAP loss. For example, the gradient w.r.t. $\vec{q}$ for the Triplet loss SH and the NT-Xent loss both have a the form $\vec{v}^{+} - \vec{v}^{-}$. The major difference between the two functions is that, for the negative candidate, the Triplet loss takes the most violating negative $\vec{v}^{-}$ while the NT-Xent loss computes a weighted sum over all negative to compute the representation of  $\vec{v}^{-}$. Therefore, the difference in evaluation performance between the Triplet loss SH and NT-Xent can only be explained by this weighted sum over all negatives. This weighted sum can be turned into a count of negatives. I.e. how many negative approximatly contribute to this weighted sum. 

How this number of candidates is counted differs per function, because each function has different characteristics. By counting the number of candidates that contribute to the gradient, we aim to get a better understanding of why a certain loss function performs better than an others.

\header{Triplet loss SH}
In Eq.~\ref{eq:tripletrad} we give the derivative of the Triplet  loss SH w.r.t $\vec{q}$.
Each query $\vec{q}$ only has a non-zero gradient when $s^{+} - s^{-} < \alpha$. If this is the case, the gradient always has the form of $\vec{v^{+}} - \vec{v^{-}}$.
For this reason, given a batch $\mathcal{B}$, the only thing we can count is the number of queries $\vec{q}$ that have a non-zero gradient:

\begin{equation}
  C^{\mathcal{B}}_{TripletSH} = \sum_{\vec{q} \in \mathcal{B}}    \mathbbm{1} \{ s^{+} - s^{-} < \alpha \},
\end{equation}

where $s^{+} = s^{0} \in \mathcal{S}_{\mathcal{P}}^{\vec{q}}$ and $s^{-} = \max \left( \mathcal{S}_{\mathcal{N}}^{\vec{q}}  \right)$. 
The Triplet loss SH takes  the maximum violating negative candidate from the negative candidate set. If the difference in similarity score between the positive and the negative candidate is bigger than $\alpha$, there is no gradient. 
We define $ C^{\mathcal{B}}_{TripletSH} $ to be \textit{the number of queries $\vec{q}$ that have a non-zero gradient given batch $\mathcal{B}$.}

\header{Triplet loss}
In Eq.~\ref{eq:tripletgrad2} we give the derivative of the Triplet  loss w.r.t $\vec{q}$. The difference with the Triplet loss SH is that the Triplet loss takes all the triplets into account that violate the distance margin $\alpha$. Therefore, we can count three things: 
\begin{enumerate}[label=(\arabic*),nosep]
	\item Per query $\vec{q}$, we can count how many triplets $\vec{v}^{+} - \vec{v}^{-}$ contribute to the gradient of that query. We define this number as $C_{Triplet}^{\vec{q}}$. 
	\item Given the entire batch $\mathcal{B}$, we can count how many triplets contribute to the gradient over the entire training batch $\mathcal{B}$. We define this number as  $C_{Triplet}^{\mathcal{B}}$.
	\item Given the entire batch $\mathcal{B}$, we can count how many queries have a gradient value of zero (i.e., no violating triplets).  We define this number as  $C_{Triplet}^{0}$:
%
\begin{subequations}
	\begin{align}
	C_{Triplet}^{\vec{q}} &= \sum_{s^{-} \in \mathcal{S}_{\mathcal{N}}^{\vec{q}}}  \mathbbm{1} \{ s^{+} - s^{-} < \alpha \}
	\\
	C_{Triplet}^{\mathcal{B}} &= \sum_{\vec{q} \in \mathcal{B}} C_{Triplet}^{\vec{q}} 
	\\
	C_{Triplet}^{0} &= \sum_{\vec{q} \in \mathcal{B}}  \mathbbm{1} \{  C_{Triplet}^{\vec{q}} = 0 \}.
	\end{align}
\end{subequations}
\end{enumerate}

\subsubsection{NT-Xent loss}

In Eq.~\ref{eq:ntxentgrad} we provide the derivative of the NT-Xent loss w.r.t $\vec{q}$.
The gradient w.r.t. query $\vec{q}$ is the difference between the positive candidate $\vec{v}^{+}$ and the weighted sum over all the negative candidates $\vec{v}^{-}$ in the batch $\mathcal{B}$.
Given a query $\vec{q}$, the positive candidate $\vec{v}^{+}$ is weighted by the factor $  \left( 1 - \frac{\exp(s_{+}/\tau)}{Z(\vec{q})} \right) $.
Each negative  $\vec{v}^{-}$ candidate is weighted by the factor $ \frac{\exp(s^{-}/\tau)}{Z(\vec{q})}$.

This means that, in principle, all the negatives and the positive candidate contribute to the gradient w.r.t $\vec{q}$. 
However, in practice most similarity scores $s^{-} \in \mathcal{S}_{\mathcal{N}}^{\vec{q}}$, for a negative candidate, will have a low value and therefore the weight value of this negative candidate in the gradient computation will be close to 0.

To count the  number of negative candidates that contribute to the gradient, we define a threshold value $\epsilon$.  
If the weight value of a negative candidate $\vec{v}^{-}$ is below this  threshold value $\epsilon$, we assume that the contribution to the gradient is negligible.
It should be noted that all candidate vectors are normalized. 
As a result, there is no additional weighting effect by the magnitude of the vector. 

For the NT-Xent loss we define three terms: $C_{NTXent}^{\vec{qv}^{-}} $, $W_{NTXent}^{\vec{qv}^{-}}$ and $W_{NT-Xent}^{\vec{qv}^{+}}$:
\begin{enumerate}[leftmargin=*,nosep,label=(\arabic*)]
\item Given a query $\vec{q}$, $C_{NT-Xent}^{\vec{qv}^{-}}$ is the number of negative candidates $\vec{v}^{-}$ that contribute to the gradient w.r.t $\vec{q}$:
\begin{equation}
	C_{NT-Xent}^{\vec{qv}^{-}}= \sum_{s^{-} \in  \mathcal{S}_{\mathcal{N}}^{\vec{q}}} \mathbbm{1} \left\{ \frac{\exp(s^{-}/\tau)}{Z(\vec{q})}  > \epsilon \right\}.
\end{equation}
We count all the negative candidates $\vec{v}^{-}$ that have a normalized similarity score with the query higher than $\epsilon$.
\item Given $C_{NT-Xent}^{\vec{qv}^{-}}$, we want to compute the sum of the weight values of the contributing negative canidates $\vec{v}^{-}$, which we define as $W_{NT-Xent}^{\vec{qv}^{-}}$:
\begin{equation}
W_{NT-Xent}^{\vec{qv}^{-}} =  \sum_{s^{-} \in  \mathcal{S}_{\mathcal{N}}^{\vec{q}}} \mathbbm{1} \left\{ \frac{\exp(s^{-}/\tau)}{Z(\vec{q})}  > \epsilon \right\}  \frac{\exp(s^{-}/\tau)}{Z(\vec{q})}.
\end{equation}
\item We define $W_{NT-Xent}^{\vec{qv}^{+}}$ as the mean weight value of the positive candidates in batch $\mathcal{B}$:
\begin{equation}
W_{NT-Xent}^{\vec{qv}^{+}}	= \frac{1}{N} \sum_{\vec{q} \in \mathcal{B}}  \left( 1 -  \frac{\exp(s^{+}/\tau)}{Z(\vec{q})} \right).
\end{equation}
\end{enumerate}
We define these two extra terms because for the NT-Xent function we have to count the candidates with a weight value above the threshold $\epsilon$. 
However, this count on its own does not provide a good picture of the contribution of these candidates to the gradient. 
Therefore, we have to compute a mean value of those weight values as well, to provide a better insight on the number of the samples were the gradient w.r.t. $\vec{q}$ is based on.

\header{SmoothAP loss}
In Eq. \ref{eq:smooth_der} we provide the derivative of the SmoothAP loss w.r.t $\vec{q}$.
The gradient w.r.t. $\vec{q}$ is a sum over tuples $\vec{v}_{i} - \vec{v}_{j}$. 
Each  tuple $\vec{v}_{i} - \vec{v}_{j}$ is weighted by the factor $sim(D_{ij})$. 
This factor $sim(D_{ij})$ gives an indication of how close the similarity score (with the query) of candidate $\vec{v}_{i}$  is compared to the similarity score of $\vec{v}_{j}$.
If the similarity scores are far apart, then $sim(D_{ij})$ will have a value close to zero. 
Therefore, we define a threshold value $\epsilon$ again. 
If the value of $sim(D_{ij})$ is lower than the threshold value, we consider the contribution of this triplet to the negligible. 
We can define $C_{Smooth}^{\vec{q}}$, which \textit{is the number of triplets $\vec{v}^{+} - \vec{v}^{-}$ that contribute to the gradient w.r.t. $\vec{q}$}, for SmoothAP as follows:
%
\begin{equation}
C_{Smooth}^{\vec{q}} = \frac{1}{|\mathcal{S}_{\mathcal{P}}^{\vec{q}}|} \sum_{i \in \mathcal{S}_{\mathcal{P}}^{\vec{q}}}  \left(\sum_{j \in \mathcal{S}_{\mathcal{N}}^{\vec{q}}}  \mathbbm{1} \{ sim(D_{ij}) > \epsilon\} +  \sum_{j \in \mathcal{S}_{\mathcal{P}}^{\vec{q}}, j \neq i}  \mathbbm{1} \{ sim(D_{ij}) > \epsilon\} \right).
\end{equation}
%
However, all triplets are also weighted by $\frac{1}{\mathcal{R}(i, \mathcal{S}_{\Omega}^{\vec{q}})^{2}}$, which is always lower than or equal to 1. Therefore, $C_{Smooth}^{\vec{q}}$ which takes the total ranking of the candidate $i$ into account, has the following form:
%
\begin{equation}
C_{Smooth}^{\vec{q}} = \frac{1}{|\mathcal{S}_{\mathcal{P}}^{\vec{q}}|} \sum_{i \in \mathcal{S}_{\mathcal{P}}^{\vec{q}}} \left(\sum_{j \in \mathcal{S}_{\mathcal{N}}^{\vec{q}}}  \mathbbm{1} \left\{ \frac{sim(D_{ij})}{\mathcal{R}(i, \mathcal{S}_{\Omega}^{\vec{q}})^{2}} > \epsilon\right\} 
+ \sum_{j \in \mathcal{S}_{\mathcal{P}}^{\vec{q}}, j \neq i}  \mathbbm{1} \left\{ \frac{sim(D_{ij})}{\mathcal{R}(i, \mathcal{S}_{\Omega}^{\vec{q}})^{2}} > \epsilon\right\} \right).
\end{equation}
%
We ignore the terms $\mathcal{R}\left(i, \mathcal{S}_{\mathcal{P}}^{\vec{q}} \right)$ and  $1 - \mathcal{R}\left(i, \mathcal{S}_{\mathcal{N}}^{\vec{q}} \right)$ for this gradient computation. 

We also count all the queries $\vec{q}$ within batch $\mathcal{B}$ which do not have a gradient value. We define this number as $C_{Smooth}^{0}$:
%
\begin{equation}
	C_{Smooth}^{0} = \sum_{\vec{q} \in \mathcal{B}} \mathbbm{1} \{ C_{Smooth}^{\vec{q}} = 0 \}.
\end{equation}
  

==> sections/old_sections/method/loss_functions.tex <==
% !TEX root =  ../../main.tex 

\subsection{Loss functions}

During training, unless otherwise stated, we iterate over the captions in $\mathcal{D}$. We randomly sample  $n$ captions and their matching images which form batch $\mathcal{B}$, therefore $|\mathcal{B}| = 2n$. All sampled images and captions will function both as queries and candidates.

\header{Triplet loss with semi hard-negative mining}
The Triplet loss is commonly used as loss function for \ac{ICR} methods \cite{faghri2018vse++, li2019vsrn, lee2018stacked, messina2021transformer, diao2021similarity, chen2020intriguing}. The \emph{Triplet loss with semi-hard negative mining} (Triplet loss SH), for a query $\vec{q}$ is defined as:
%
\begin{equation}
	\mathcal{L}_\mathit{TripletSH}^{\vec{q}} = \max(\alpha - s^{+} +  s^{-}, 0),
\end{equation}
%
where $\alpha$ serves as a margin parameter, $s^{-} = \max(S_{\mathcal{N}}^{\vec{q}} )$ and   $s^{+} =  s_{0} \in S_{\mathcal{P}}^{\vec{q}}$. 
Note that here $\mathcal{S}_{\mathcal{P}}^{\vec{q}}$ only contains one element per query, therefore we take $s_{0}$ from $ S_{\mathcal{P}}^{\vec{q}}$. The Triplet loss SH over the entire training batch is defined as:
%
\begin{equation}
\mathcal{L}_\mathit{TripletSH}= \sum_{\vec{q} \in \mathcal{B}} 	\mathcal{L}_\mathit{TripletSH}^{\vec{q}}.
\end{equation}
%
Triplet loss SH performs a form of soft-negative mining per query by selecting the negative candidate with the highest similarity score w.r.t.\ the query, we also refer to this as the maximum violating query. For computational efficiency, this soft-negative mining is executed within the context of the training batch $\mathcal{B}$ and not over the entire training set.  For this reason it is called \emph{semi hard-negative mining}. 

Instead of the definition just given, another possibility is to take the Triplet-loss over all triplets in the batch $\mathcal{B}$. 
This is the definition of the standard \emph{Triplet-loss} \citep{kiros2014unifying}:
%
\begin{subequations}
	\begin{align}
	\mathcal{L}_\mathit{Triplet}^{q} &= \sum_{ s^{-} \in S_{\mathcal{N}}^{q }}\max(\alpha - s^{+} +  s^{-}, 0)
	\\
	\mathcal{L}_\mathit{Triplet} &= \sum_{\vec{q} \in \mathcal{B}} 	\mathcal{L}_\mathit{Triplet}^{\vec{q}}.
	\end{align}
\end{subequations}

\paragraph{Gradient w.r.t. $\vec{q}$}
\label{par:gradtriplet}
We give the form of the gradient of $\mathcal{L}_\mathit{triplet SH}^{q} $ w.r.t. $\vec{q}$. By doing this we can analyze what the form is of the update  w.r.t. $\vec{q}$ looks like:
%
\begin{equation} \label{eq:tripletrad}
	\frac{\partial \mathcal{L}_\mathit{TripletSH}^{\vec{q}}}{\partial \vec{q}} = 
	\left\{
	\begin{array}{ll}
	\vec{v}^{+} - \vec{v}^{-}, & \textrm{if } s^{+} -  s^{-} < \alpha\\
	0, & \textrm{otherwise}.
	\end{array}
	\right.
\end{equation}
%
Based on Eq.~\ref{eq:tripletrad}, the gradient w.r.t. $\vec{q}$ is the difference between the representation of the positive and of the negative candidate. There is only a gradient value when $s^{+} - s^{-} < \alpha$, due to the $max(0, \dots)$, and the  value of the gradient is  independent of $s^{+} - s^{-} < \alpha$. 

The gradient of $\mathcal{L}_\mathit{Triplet}^{\vec{q}} $ w.r.t. $\vec{q}$ has a similar form. However, there the gradients is a sum over all triplets that violate $s^{+} +  s^{-} < \alpha$:
%
\begin{equation}\label{eq:tripletgrad2}
	\frac{\partial \mathcal{L}_\mathit{Triplet}^{\vec{q}}}{\partial \vec{q}} = \sum_{\vec{v}^{-} \in \mathcal{N}_{\vec{q}}}  \mathbbm{1} \{s^{+} - s^{-} < \alpha \} \left( 	\vec{v}^{+} - \vec{v}^{-} \right).
\end{equation}
%
Based on Eq.~\ref{eq:tripletrad}  and~\ref{eq:tripletgrad2} it becomes clear that the gradients w.r.t $\vec{q}$ for $ \mathcal{L}_\mathit{TripletSH}$ and $ \mathcal{L}_\mathit{Triplet}$ have a similar form, the only difference is the number of triplets that is taken into account when computing the gradient.

\header{NT-Xent loss}
% Cite \cite{zhang2018deep}
The \emph{NT-Xent loss} \cite{chen2020simple} is a loss function commonly used in the field of self-supervised representation learning \cite{oord2018representation, chen2020simple}. A similar function has also been proposed by \citet{zhang2018deep} in the context of \ac{ICR}.
The NT-Xent loss is defined as: 
%
\begin{equation} \label{eq:ntxent}
	\mathcal{L}_\mathit{NT\mbox{-}Xent} =- \frac{1}{2n} \sum_{\vec{q} \in \mathcal{B}} \log \frac{\exp({s^{+}/ \tau )}}{ \sum_{
s_{i} \in \mathcal{S}_{\Omega}^{\vec{q}}
}^{} \exp({s_{i}/ \tau ) }},
\end{equation}
%
where $\tau$ functions as temperature parameters. As for the Triplet-loss formulation: $s^{+} =  s_{0} \in S_{\mathcal{P}}^{\vec{q}}$. 
The major difference with the Triplet-loss SH is that the NT-Xent loss takes the entire negative candidate set into account. 

\paragraph{Gradient w.r.t. $\vec{q}$}\label{par:gradntxent}

The gradient w.r.t.\ $\vec{q}$ for the NT-Xent loss is defined as:
%
\begin{equation}
\frac{\partial \mathcal{L}_\mathit{NT\mbox{-}Xent}^{\vec{q}}}{\partial \vec{q}} = 
  \left( 1 - \frac{\exp(s^{+}/\tau)}{Z(\vec{q})} \right)/ \tau \vec{v}^{+} -  \sum_{s^{-} \in S_{\mathcal{N}}^{q }} \frac{\exp(s^{-}/\tau)}{Z(\vec{q})}  \tau \vec{v}^{-},
\label{eq:ntxentgrad}
\end{equation}
%
where $Z(\vec{q}) =   \sum_{s_{i} \in \mathcal{S}_{\Omega}^{\vec{q}}}^{} \exp({s_{i}/ \tau ) }$, a normalization constant depending on $\vec{q}$. 
When looking at Eq.~\ref{eq:ntxentgrad}, it is clear that the gradient w.r.t.\ $\vec{q}$ is the weighted difference of the positive  candidate $\vec{v}^{+}$ and the weighted sum over all the negative candidates, $\vec{v}^{-} \in \mathcal{N}_{\vec{q}}$, in the training batch. 

The weight for each candidate is based on the similarity with the query, normalized over the sum of the similarities of all candidates. 
This is in contrast with the Triplet-loss (Eq.~\ref{eq:tripletrad}), where all candidates are weighted equally. 
As also argued by \citet{chen2020simple}, the NT-Xent loss performs a natural form of (hard) negative weighting. 
The more similar a negative is to the query, the higher the weight of this negative in the gradient computation. 
%It should be noted that  $\left( 1 - \frac{\exp(s^{+}/\tau)}{Z(\vec{q})} \right) = \sum_{s^{-} \in S_{\mathcal{N}}^{q }} \frac{\exp(s^{-}/\tau)}{Z(\vec{q})} $, hence the positive candidate $\vec{v}^{+}$  has the same weight value as the sum of the weights over all the negative candidates, $\vec{v}^{-}  \in \mathcal{N}^{\vec{q}}$.

\header{SmoothAP loss}
The average precision metric w.r.t.\ a query $\vec{q}$ and candidate set $\Omega$ is defined as:
%
\begin{equation}\label{eq:ap}
	AP_{\vec{q}} = 
	\frac{1}{|\mathcal{S}_{\mathcal{P}}^{\vec{q}}|} 
	\sum_{i \in \mathcal{S}_{\mathcal{P}}^{\vec{\vec{q}}}} 
	\frac{\mathcal{R}(i, \mathcal{S}_{\mathcal{P}}^{\vec{q}})}
	{\mathcal{R}(i, \mathcal{S}_{\Omega}^{\vec{q}})},
\end{equation} 
%
where $\mathcal{R}(i, \mathcal{S})$ is a function that returns the ranking of candidate $i \in \mathcal{S}$. $\mathcal{R}(i,\mathcal{S})$ is defined as:
%
\begin{equation}
	\mathcal{R}(i, \mathcal{S}) = 1 + \sum_{j \in \mathcal{S}, i \neq j} \mathbbm{1} \{s_{i} - s_{j} < 0 \}.
\end{equation}
%
The problem is that the indicator function $\mathbbm{1} \{\cdot\}$ is non-differentiable.  
Let us introduce the matrix $D$, defined as:
%
\begin{equation}
D = \begin{bmatrix} 
s_{1}    &  \dots   & s_{m} \\
\vdots   &  \ddots  & \vdots \\ 
s_{1}    &  \dots   & s_{m} 
\end{bmatrix}
- 
\begin{bmatrix} 
s_{1}   &  \dots   &   s_{1} \\
\vdots  &  \ddots  &   \vdots \\
s_{m}   &  \dots   &   s_{m} 
\end{bmatrix}.
\end{equation}
%
By using the matrix $D$, Eq.~\ref{eq:ap} can be written as follows:
%
\begin{equation} 
AP_{\vec{\vec{q}}} = {}
 \frac{1}{|\mathcal{S}_{\mathcal{P}}^{\vec{q}}|} \!\sum_{\substack{i\in\mathcal{S}_{\mathcal{P}}^{\vec{q}}}} \!
\frac{1+ \sum_{j \in \mathcal{S}_{\mathcal{P}} ,j\neq i} \mathbbm{1}\{D_{ij} > 0\}}
{1+ \sum_{j\in \mathcal{S}_{\mathcal{P}}^{\vec{q}} ,j\neq i} \mathbbm{1}\{D_{ij} > 0\} 
+ \sum_{j\in \mathcal{S}_{\mathcal{N}}^{\vec{q}} } \mathbbm{1}\{D_{ij} > 0\}}.
\nonumber
\end{equation}
%
The indicator function is still not differentiable. 
To overcome this problem, the indicator function can be replaced by a sigmoid function:
%
\begin{equation} \label{eq:der_sig}
 \mathcal{G}(x; \tau) = \frac{1}{1 + e^{\frac{-x}{\tau}}}.
\end{equation}
%
By replacing the indicator function $\mathbbm{1} \{\cdot\}$  by $\mathcal{G}$,  the Average Precision metric can be approximated with a smooth function:
%
\begin{equation}  \label{eq:smooth}
AP_{\vec{q}} \approx {}
	\frac{1}{|\mathcal{S}_{\mathcal{P}}^{q}|} \sum_{i\in\mathcal{S}_{\mathcal{P}}^{\vec{q}}} 
	\frac{1 + \sum_{j \in \mathcal{S}_{\mathcal{P}}^{\vec{q}} , j\neq i} \mathcal{G}(D_{ij}; \tau)}
	 {1 + \sum_{j\in \mathcal{S}_{\mathcal{P}}^{\vec{q}}, j\neq i} \mathcal{G}(D_{ij}; \tau) 
		+ \sum_{j\in \mathcal{S}_{\mathcal{N}}^{\vec{q}}} \mathcal{G}(D_{ij}; \tau)}.
\nonumber		
\end{equation}
%
This loss function is called SmoothAP and has been introduced by \citet{brown2020smooth} in the context of image retrieval. 
The total loss over a batch $\mathcal{B}$ can then be formulated as follows: 
% 
\begin{equation}
\mathcal{L}_{AP}  = \frac{1}{|\mathcal{B}|}\sum_{\vec{q} \in \mathcal{B}} (1 - AP_\vec{q}).
\end{equation}

\paragraph{Gradient w.r.t. $\vec{q}$}\label{par:gradsmooth} 

In\footnote{\url{}} we provide the full derivation of the gradient of SmoothAP w.r.t. $\vec{q}$. We introduce $sim(D_{ij}$, which is the derivative of  \label{eq:der_sig}.
%
\begin{equation}\label{eq:smooth_der}
\resizebox{\textwidth}{!}{$
\frac{\partial AP_{\vec{q}}}{\partial \vec{q}} = {}
 \frac{1}{|\mathcal{S}_{\mathcal{P}}^{\vec{q}}|} \sum_{\substack{i\in\mathcal{S}_{\mathcal{P}}^{\vec{q}}}} \frac{1}{ \mathcal{R}\left(i, \mathcal{S}_{\Omega}^{\vec{q}}\right) ^{2}} 
\quad\mathcal{R}\left(i, \mathcal{S}_{\mathcal{P}}^{\vec{q}}\right)
\left( \sum_{j\in \mathcal{S}_{\mathcal{N}}^{\vec{q}}} sim(D_{ij})  ( \vec{v}_{i} - \vec{v}_{j}) \right)
-  
\quad \left( \mathcal{R}\left(i, \mathcal{S}_{\mathcal{N}}^{\vec{q}}\right) - 1 \right) 
\left( \sum_{j\in \mathcal{S}_{\mathcal{P}}^{\vec{q}}, j\neq i}  sim(D_{ij})  ( \vec{v}_{i} - \vec{v}_{j}) \right).
$}
\end{equation}
%

Given Eq.~\ref{eq:smooth_der}, it is less trivial to infer what the update w.r.t.\ $\vec{q}$ looks like in terms of positive candidates $\vec{v}_{i}$ and negative candidates $\vec{v}_{j}$. However, we can derive the following two properties:

\begin{enumerate}[leftmargin=*,nosep,label=(\arabic*)]
	\item The lower a positive candidate $\vec{v}_{i}$ is in the total ranking, the less this candidate is taken into account for the gradient computation w.r.t.\ $\vec{q}$, due the inverse quadratic term $\frac{1}{ \mathcal{R}\left(i, \mathcal{S}_{\Omega}^{q}\right) ^{2}} $. This is in line with optimizing the AP as a metric, because positive candidates that are ranked low contribute less to the total AP score, and therefore are less important to optimize.
	\item Each triplet weighted according to their difference is similarity score $D_{ij}$. If their different is similarity score w.r.t.\ query $\vec{q}$ is relatively small (i.e., $D_{ij}$ is close to zero), $sim(D_{ij})$ will have a high value. This is because $sim(D_{ij})$  is the derivative of the sigmoid function (see Appendix \ref{appendix:1} for details).  This is also in line with the SmoothAP loss because we use a sigmoid to simulate the step-function; only triplets of candidates that have a similar similarity score will have a non-zero gradient. 
\end{enumerate} 

\header{Implementation of SmoothAP for ICR}
By using the SmoothAP loss, we can directly optimize a ranking metric over the candidate set. We can benefit from the fact that $S_{\mathcal{P}}^{q}$ can contain multiple candidates per query because each tuple $i \in \mathcal{D}$ contains one image and $k$ captions. 
As a result, we have to iterate over the images per training epoch instead of the captions (as opposed to the Triplet and the NT-Xent loss).  Therefore, for each image query $\vec{q}$, $|\mathcal{S}_{\mathcal{P}}| = k$. For $\mathcal{S}_{\mathcal{N}}$, we use all the captions from the other images in the training batch. 
When optimizing using the SmoothAP loss, the batch size is $|\mathcal{B}| = n(k + 1)$, where $n$ is the number of images in the batch. If we optimize for the \acf{t2i}-task, we still use the SmoothAP loss as optimization function. 
However, we only have one positive candidate per caption. Therefore, we optimize a top-1 ranking instead of a top-$k$ ranking, which is the case for \ac{i2t}.


==> sections/old_sections/method/method.tex <==
% !TEX root =  ../../main.tex 

\section{Method}\label{sec:method}

In this section, we detail the loss functions that we evaluate in this work in the context of \acl{ICR}.
We give the form of the gradient of each loss function w.r.t. query $\vec{q}$ to analyze how many samples contribute to the update of the network w.r.t. $\vec{q}$. 
Using this analysis, we want to answer the question why one loss function results in better evaluation performance than others.

\input{sections/method/notation.tex}

\input{sections/method/loss_functions.tex}

\input{sections/method/grad_count.tex}

==> sections/old_sections/method/notation.tex <==
% !TEX root =  ../../main.tex 

\subsection{Task definition, notation and formulation}

We closely follow the notation introduced in \citep{brown2020smooth,chen2020simple,varamesh2020self}.

\header{Notation and task definition}
We start with a multi-modal image-caption dataset $\mathcal{D} = \{(\textbf{x}_{I}^{i}, \textbf{x}_{C_1}^{i}$, \dots, $\textbf{x}_{C_k}^{i})^{i}, \dots \}_{i=1}^{N}$  that contains $N$ image-caption tuples. 
For each image $\textbf{x}_{I}^{i}$, we have $k$ corresponding captions $\textbf{x}_{C_1}^{i}, \dots, \textbf{x}_{C_k}^{i}$, that describe the scene depicted in image $i$.  
All captions in the same tuple $i$ are considered as \textit{positive} or \textit{matching} captions w.r.t. image $\textbf{x}_{I}^{i}$ and the other way around.

In the \ac{ICR} task, either an image or a caption can function as a query. 
Given a query $\vec{q}$, the task is to rank all candidates in a candidate set $\Omega = \{\vec{v}_{i} \mid i=0, \dots, m\}$. 
A positive, e.g. matching, candidate is denote as $\vec{v}^{+}$ and a negative candidate as $\vec{v}^{-}$.
For each query $\vec{q}$, we can split the candidate set $\Omega$ into two disjoint subsets: $ \vec{v}^{+} \in \mathcal{P}_{\vec{q}}$  and $  \vec{v}^{-} \in\mathcal{N}_{\vec{q}}$. 
$\mathcal{P}_{\vec{q}}$  is called the \textit{positive} candidate set and contains the positive candidates, from the same tuple (but from the other modality) $i \in \mathcal{D}$ as query $\vec{q}$.
$\mathcal{N}_{\vec{q}}$ is called the \textit{negative} candidate set and contains all negative $ \vec{v}^{-}$, where $\{   \vec{v}^{-}  \mid   \vec{v}^{-} \in \Omega,   \vec{v}^{-}  \notin  \mathcal{P}_{\vec{q}} \}$. 
We assume a binary match between images and captions, they either match or they do not match. 

The set with similarity scores for each $\vec{v}_{i} \in \Omega$ w.r.t. query $\vec{q}$ is defined as:
%
\begin{equation}
	\mathcal{S}_{\Omega}^{\vec{q}} = \left\{ s_{i} = \left\langle \frac{\vec{q}}{\| \vec{q}\|}  \frac{\vec{v}_{i}}{\| \vec{v}_{i }\|} \right\rangle, i=0,\dots, m \right\}.
\end{equation}
%
We use cosine similarity as a similarity scoring function.  
$S_{\Omega}^{\vec{q}}$ consists of two disjoint subsets: $S_{\mathcal{P}}^{\vec{q}}$ and $S_{\mathcal{N}}^{\vec{q}}$.  $S_{\mathcal{P}}^{\vec{q}}$ contains the similarity scores for the positive candidates and $S_{\mathcal{N}}^{\vec{q}}$ the similarity scores for the negative candidates. 

The \ac{ICR} task can be subdivided into two sub-taks: \acfi{i2t} retrieval and \acfi{t2i} retrieval.
For the \ac{i2t} task, an image is presented as a query and the task is then to rank a candidate set of captions based on their similarity w.r.t. the query image. 
For the \ac{t2i} task a caption functions as the query and the candidate set consists of images.
To compute the image and caption representation we  define two encoders, an \textit{image} and a \textit{caption}  encoder, which do not share parameters. 


==> sections/old_sections/related_work-v2.tex <==
% !TEX root =  ../main.tex 

\section{Related Work}
\label{section:related}

In this section we first provide a brief overview of the benchmark methods we use in this work (Section \ref{section:related_benchmark}) and what happend in the \ac{ICR} field after these two benchmark methods have been published (Section \ref{section:related_after}). Next, we give an overview of representation learning in relation to \ac{ICR} (Section \ref{section:related_metric}). 

\subsection{Image-caption retrieval}

To remain focused, we target specific~\ac{ICR} methods that are optimized for the \ac{ICR}-task only and satisfy three criteria: 
\begin{enumerate}[label=(\arabic*)]
	\item The methods we use have solely been trained and evaluated on the same benchmark dataset.
	This means that no additional pre-training on a different dataset (or task) has been applied when optimizing the method. 
	However, this does not imply that some of the method components (i.e., the image encoders) have not already been pre-trained on a different task. 
	\item  The \ac{ICR} methods we use are global matching methods. 
	Global matching methods are methods that compute one global representation for both the entire input image and the full caption. 
	\item  The methods do not require any additional supervision signal besides the contrastive loss for optimization.
\end{enumerate}

\subsubsection{VSE++ and VSRN}
\label{section:related_benchmark}

In this work we evaluate two \ac{ICR} methods with different loss functions: VSE++ \cite{ faghri2018vse++} and VSRN \cite{li2019visual}. 

VSE++ has been introduced by \citet{faghri2018vse++}.
For the image encoder two different CNNs are used (VGG19~\citep{simonyan2014very} and ResNet-152~\citep{he2016deep}) to compute a global image representation.
The caption encoder is a single directed LSTM-based encoder. 
The major contribution of \citet{faghri2018vse++} is the introduction of the notion of mining semi hard-negative triplets for the \ac{ICR} task.
By using the hardest negative in the batch for each positive pair, their method outperforms state-of-the-art methods that do not apply this semi-hard negative mining. 

VSRN, introduced by \citet{li2019visual}, takes a set of pre-computed image region features as input. 
A Graph Convolutional Network \cite{kipf2016semi} is used to enhance the relationships between each region vector.
Finally, the sequence of region feature vectors is put through an RNN network to encode the global image representation.
VSRN uses the same caption encoder and the same loss as \cite{faghri2018vse++}.

Both VSE++ and VSRN are solely optimized and evaluated on the Flickr30k \cite{young2014image} and MS-COCO \cite{lin2014microsoft} datasets, are optimized with the Triplet-loss with semi-hard negative mining and compute a global representation for both the image and the caption. 

\subsubsection{After VSE++ and VSRN}
\label{section:related_after}

After VSE++ and VSRN, the SGRAF \cite{diao2021similarity}  and IMRAM \cite{chen2020imram} methods have been introduced. We do not use these two methods for our study because they either do not outperform VSRN \cite{chen2020imram} or rely on similar method principles as the VSRN method \cite{diao2021similarity}.
The main recent progress in the \ac{ICR} field has been characterized by a shift towards transformer-based  \cite{vaswani2017attention}  methods, both for the image and caption encoder.  
To the best of our knowledge TREN \cite{messina2021transformer}, VisualSparta \cite{luvisualsparta} and TERAN \cite{messina2020fine} are the only transformer-based \ac{ICR} methods that are solely optimized using MS-COCO  \cite{lin2014microsoft}  or Flickr30k \cite{young2014image}.
Other methods such as OSCAR \cite{li2020oscar}, UNITER \cite{chen2020uniter}, Vilbert \cite{lu2019vilbert} and ViLT-B \cite{kim2021vilt} either use additional data sources and/or loss functions to train the methods.
Besides that, these methods do not solely focus on the \ac{ICR} task, but on a wide variety of vision-language tasks such as visual QA, captioning, and retrieval.

Recently, much progress in \ac{ICR}, and multi-modal matching in general, has been driven by the vast amount of data used for training the \ac{ICR} methods, for example, CLIP \cite{radford2021learning} and Align \cite{jia2021scaling}. 
CLIP~\citep{radford2021learning} is trained on a dataset containing 400 million image-caption pairs, which have been scraped from public sources on the internet by using a list of 500,000 keywords. 
Align~\citep{jia2021scaling} is trained on a dataset containing 1.8 billion `noisy' image-caption pairs. 
Neither of the two datasets used for training CLIP and ALIGN is publicly available. 
For comparison, the biggest publicly available image-caption dataset, Conceptual Captions \cite{sharma2018conceptual}, contains roughly 3.3 million image-caption pairs, which is only a fraction of the data used to train CLIP and ALIGN.

In this work, we focus on two non-transformer-based methods that do not use any additional training data besides the benchmark sets on which they are evaluated. 
This to keep the experiments in this work scalable w.r.t. training time and to eliminate the effect of additional data on the training performance.  
Since it is not always realistic to obtain more data or more compute to process the data, we believe it is important to pursue other avenues of algorithm development than simply using more data. 
We want to utilize the given benchmark sets datasets \cite{lin2014microsoft, young2014image} as optimally as possible by exploiting different optimization losses for \ac{ICR}. 

\subsection{Learning representation for ICR}
\label{section:related_metric}

The \ac{ICR} task is evaluated with the Recall@k metric.
It is non-trivial to optimize an \ac{ICR} method with Recall@k as a loss function directly, due to the non-differentiable nature of this evaluation metric.
Therefore, pair-wise loss functions like the Triplet-loss with semi-hard negative mining and NT-Xent loss are used to optimize the item representations \citep{faghri2018vse++,  li2019vsrn, messina2021transformer, diao2021similarity, lee2018stacked, chen2020intriguing, jia2021scaling}.
However,  these pair-wise loss functions do not optimize for the desired output directly  (i.e. a ranking) which could result in sub-optimal performances on the evaluation task.
To overcome the discrepancy between the training objective and the discrete evaluation metric(s), several works have introduced (smooth) approximations of non-differentiable evaluation metrics, such as Average Precision \cite{brown2020smooth, cakir2019deep} or  SmoothI \cite{thonet2021smoothi} and LambdaLoss \cite{wang2018lambdaloss} which could function as any metric approximation.

Thus far, no \ac{ICR} method has been optimized by using a smooth approximation of a ranking metric directly. 
In this work we examine if optimizing \ac{ICR} methods by using a smooth approximation of \acf{mAP}, SmoothAP \cite{brown2020smooth}, results in better evaluation performances than a standard pair-wise loss. 
SmoothAP optimizes a list-wise ranking criteria instead of a pair-wise similarity between candidates which therefore also optimizes the Recall@k. 
Besides that, SmoothAP can also utilize the fact that there are multiple captions per image in the dataset. 

The representation learning task is to learn a general representation of the data, independent of a particular task \cite{bengio2013representation}. 
Recently, a new self-supervised representation learning paradigm has been introduced which showed impressive results on several modalities like images \cite{chen2020simple, he2020momentum}, audio \cite{wang2021multi, oord2018representation} and image-text pairs \cite{radford2021learning, jia2021scaling}.
The training objective of this paradigm is to optimize the similarity between representations of similar items, which are created by augmenting a source input into two new data points, of information while minimizing the similarity of dissimilar items of information. 
The workhorse of this self-supervised learning paradigm is the NT-Xent loss \cite{chen2020simple}. 
Experimental results by \cite{chen2020simple} show that the NT-Xent loss outperforms the Triplet loss (with a large margin) and the Triplet with semi-hard negative mining on representation learning benchmark tasks.
Because the optimization objective for the \ac{ICR} task is the same as for the representation learning task, it would be a natural step forward to adopt the NT-Xent loss as the loss function for \ac{ICR} instead of the Triplet loss to improve evaluation performances without any additional costs.

Recently \citet{jia2021scaling}, adopted the NT-Xent loss for the optimization of the Align method.
However, the use of the NT-Xent loss in this work also came with a new method and a vast amount of training data and no comparison has been made with the Triplet loss with semi-hard negative mining.
Earlier, \citet{zhang2018deep} have introduced a cross-entropy based loss function  (which is relatively similar to the NT-Xent loss) for the \ac{ICR} task as well. 
Also in the work of \citet{zhang2018deep}, there is no fair comparison between the newly introduced optimization function and the Triplet loss with semi-hard negative mining. 
Therefore, is unclear how much of the evaluation metric improvement can be attributed to the use of the NT-Xent loss over the Triplet-loss with semi-hard negative mining.
In this work we compare the NT-Xent loss with the Triplet loss with semi-hard negative mining in an equal training set-up. This to examine if, or how much of, the improvement of the evaluation scores can be contributed to the use of the NT-Xent loss.


==> sections/old_sections/related_work.tex <==
% !TEX root =  ../main.tex 

\section{Related Work}
\label{section:related}

In this section we first provide a brief overview of the benchmark methods we use in this work (Section \ref{section:related_benchmark}) and what happend in the \ac{ICR} field after these two benchmark methods have been published (Section \ref{section:related_after}). Next, we give an overview of representation learning in relation to \ac{ICR} (Section \ref{section:related_metric}). 

\subsection{Image-caption retrieval}

To remain focused, we target specific~\ac{ICR} methods that are optimized for the \ac{ICR}-task only and satisfy three criteria: 
\begin{enumerate}[label=(\arabic*)]
	\item The methods we use have solely been trained and evaluated on the same benchmark dataset.
	This means that no additional pre-training on a different dataset (or task) has been applied when optimizing the method. 
	However, this does not imply that some of the method components (i.e., the image encoders) have not already been pre-trained on a different task. 
	\item  The \ac{ICR} methods we use are global matching methods. 
	Global matching methods are methods that compute one global representation for both the entire input image and the full caption. 
	\item  The methods do not require any additional supervision signal besides the contrastive loss for optimization.
\end{enumerate}

\subsubsection{VSE++ and VSRN}
\label{section:related_benchmark}

In this work we evaluate two \ac{ICR} methods with different loss functions: VSE++ \cite{ faghri2018vse++} and VSRN \cite{li2019visual}. 

VSE++ has been introduced by \citet{faghri2018vse++}.
For the image encoder two different CNNs are used (VGG19~\citep{simonyan2014very} and ResNet-152~\citep{he2016deep}) to compute a global image representation.
The caption encoder is a single directed LSTM-based encoder. 
The major contribution of \citet{faghri2018vse++} is the introduction of the notion of mining semi hard-negative triplets for the \ac{ICR} task.
By using the hardest negative in the batch for each positive pair, their method outperforms state-of-the-art methods that do not apply this semi-hard negative mining. 

VSRN, introduced by \citet{li2019visual}, takes a set of pre-computed image region features as input. 
A Graph Convolutional Network \cite{kipf2016semi} is used to enhance the relationships between each region vector.
Finally, the sequence of region feature vectors is put through an RNN network to encode the global image representation.
VSRN uses the same caption encoder and the same loss as \cite{faghri2018vse++}.

Both VSE++ and VSRN are solely optimized and evaluated on the Flickr30k \cite{young2014image} and MS-COCO \cite{lin2014microsoft} datasets, are optimized with the Triplet-loss with semi-hard negative mining and compute a global representation for both the image and the caption. 

\subsubsection{After VSE++ and VSRN}
\label{section:related_after}

After VSE++ and VSRN, the SGRAF \cite{diao2021similarity}  and IMRAM \cite{chen2020imram} methods have been introduced. We do not use these two methods for our study because they either do not outperform VSRN \cite{chen2020imram} or rely on similar method principles as the VSRN method \cite{diao2021similarity}.
The main recent progress in the \ac{ICR} field has been characterized by a shift towards transformer-based  \cite{vaswani2017attention}  methods, both for the image and caption encoder.  
To the best of our knowledge TREN \cite{messina2021transformer}, VisualSparta \cite{luvisualsparta} and TERAN \cite{messina2020fine} are the only transformer-based \ac{ICR} methods that are solely optimized using MS-COCO  \cite{lin2014microsoft}  or Flickr30k \cite{young2014image}.
Other methods such as OSCAR \cite{li2020oscar}, UNITER \cite{chen2020uniter}, Vilbert \cite{lu2019vilbert} and ViLT-B \cite{kim2021vilt} either use additional data sources and/or loss functions to train the methods.
Besides that, these methods do not solely focus on the \ac{ICR} task, but on a wide variety of vision-language tasks such as visual QA, captioning, and retrieval.

Recently, much progress in \ac{ICR}, and multi-modal matching in general, has been driven by the vast amount of data used for training the \ac{ICR} methods, for example, CLIP \cite{radford2021learning} and Align \cite{jia2021scaling}. 
CLIP~\citep{radford2021learning} is trained on a dataset containing 400 million image-caption pairs, which have been scraped from public sources on the internet by using a list of 500,000 keywords. 
Align~\citep{jia2021scaling} is trained on a dataset containing 1.8 billion `noisy' image-caption pairs. 
Neither of the two datasets used for training CLIP and ALIGN is publicly available. 
For comparison, the biggest publicly available image-caption dataset, Conceptual Captions \cite{sharma2018conceptual}, contains roughly 3.3 million image-caption pairs, which is only a fraction of the data used to train CLIP and ALIGN.

In this work, we focus on two non-transformer-based methods that do not use any additional training data besides the benchmark sets on which they are evaluated. 
This to keep the experiments in this work scalable w.r.t. training time and to eliminate the effect of additional data on the training performance.  
Since it is not always realistic to obtain more data or more compute to process the data, we believe it is important to pursue other avenues of algorithm development than simply using more data. 
We want to utilize the given benchmark sets datasets \cite{lin2014microsoft, young2014image} as optimally as possible by exploiting different optimization losses for \ac{ICR}. 

\subsection{Learning representation for ICR}
\label{section:related_metric}

The \ac{ICR} task is evaluated with the Recall@k metric.
It is non-trivial to optimize an \ac{ICR} method with Recall@k as a loss function directly, due to the non-differentiable nature of this evaluation metric.
Therefore, pair-wise loss functions like the Triplet-loss with semi-hard negative mining and NT-Xent loss are used to optimize the item representations \citep{faghri2018vse++,  li2019vsrn, messina2021transformer, diao2021similarity, lee2018stacked, chen2020intriguing, jia2021scaling}.
However,  these pair-wise loss functions do not optimize for the desired output directly  (i.e. a ranking) which could result in sub-optimal performances on the evaluation task.
To overcome the discrepancy between the training objective and the discrete evaluation metric(s), several works have introduced (smooth) approximations of non-differentiable evaluation metrics, such as Average Precision \cite{brown2020smooth, cakir2019deep} or  SmoothI \cite{thonet2021smoothi} and LambdaLoss \cite{wang2018lambdaloss} which could function as any metric approximation.

Thus far, no \ac{ICR} method has been optimized by using a smooth approximation of a ranking metric directly. 
In this work we examine if optimizing \ac{ICR} methods by using a smooth approximation of \acf{mAP}, SmoothAP \cite{brown2020smooth}, results in better evaluation performances than a standard pair-wise loss. 
SmoothAP optimizes a list-wise ranking criteria instead of a pair-wise similarity between candidates which therefore also optimizes the Recall@k. 
Besides that, SmoothAP can also utilize the fact that there are multiple captions per image in the dataset. 

The representation learning task is to learn a general representation of the data, independent of a particular task \cite{bengio2013representation}. 
Recently, a new self-supervised representation learning paradigm has been introduced which showed impressive results on several modalities like images \cite{chen2020simple, he2020momentum}, audio \cite{wang2021multi, oord2018representation} and image-text pairs \cite{radford2021learning, jia2021scaling}.
The training objective of this paradigm is to optimize the similarity between representations of similar items, which are created by augmenting a source input into two new data points, of information while minimizing the similarity of dissimilar items of information. 
The workhorse of this self-supervised learning paradigm is the NT-Xent loss \cite{chen2020simple}. 
Experimental results by \cite{chen2020simple} show that the NT-Xent loss outperforms the Triplet loss (with a large margin) and the Triplet with semi-hard negative mining on representation learning benchmark tasks.
Because the optimization objective for the \ac{ICR} task is the same as for the representation learning task, it would be a natural step forward to adopt the NT-Xent loss as the loss function for \ac{ICR} instead of the Triplet loss to improve evaluation performances without any additional costs.

Recently \citet{jia2021scaling}, adopted the NT-Xent loss for the optimization of the Align method.
However, the use of the NT-Xent loss in this work also came with a new method and a vast amount of training data and no comparison has been made with the Triplet loss with semi-hard negative mining.
Earlier, \citet{zhang2018deep} have introduced a cross-entropy based loss function  (which is relatively similar to the NT-Xent loss) for the \ac{ICR} task as well. 
Also in the work of \citet{zhang2018deep}, there is no fair comparison between the newly introduced optimization function and the Triplet loss with semi-hard negative mining. 
Therefore, is unclear how much of the evaluation metric improvement can be attributed to the use of the NT-Xent loss over the Triplet-loss with semi-hard negative mining.
In this work we compare the NT-Xent loss with the Triplet loss with semi-hard negative mining in an equal training set-up. This to examine if, or how much of, the improvement of the evaluation scores can be contributed to the use of the NT-Xent loss.


==> sections/old_sections/results.tex <==
% !TEX root =  ../main.tex 
\section{Results}\label{sec:results}

\subsection{Which loss function results in the best ICR evaluation performance?}


\input{tables/flickr/table.tex}
\input{tables/ms-coco/table.tex}

In this section we compare the four different loss functions we described in Section~\ref{sec:method} for the \ac{ICR} task, on two methods \cite{faghri2018vse++, li2019vsrn} and two benchmark sets \cite{lin2014microsoft, young2014image}. 
See Table~\ref{table:f30k} and~\ref{table:coco} for the experimental results.
Based on the tables, we have the following observations:

\begin{enumerate}[label=(\roman*)]
	\item Given a  fixed method and the default hyper-parameter for each loss function, the Triplet loss SH overall results in the best evaluation scores, regardless of the dataset, method or task. 
	\item Similar to the findings of \cite{faghri2018vse++}, we find that the Triplet loss SH consistently outperforms the general Triplet loss, which takes all the negative triplets in the batch into account that violate the margin constraint.
	\item The NT-Xent loss consistently underperforms compared to the Triplet loss SH. This is in contrast with findings of \cite{chen2020simple}, that show that the NT-Xent loss results in better down-stream evaluation performances on a (augmented image-to-image) representation learning task, compared to the Triplet loss SH. 
	Although the \ac{ICR} task has different (input) data-modalities, the underlying learning object is the same for \ac{ICR} and augmented image-to-image representation learning (i.e., contrasting positive and negative pairs). 
	\item Only for the VSE++ method on the \ac{i2t} task, SmoothAP performs similar to the Triplet-loss SH.
	\item SmoothAP does not outperform the Triplet loss SH. This is in contrast with the findings of \cite{brown2020smooth}, where SmoothAP does outperform Triplet-loss SH and other metric learning functions.
	\item The method with the best Recall@k score also has the highest mAP@k score. 
\end{enumerate} 
 
\noindent%
Based on our observations in Table~\ref{table:f30k} and~\ref{table:coco} we conclude the following:
\begin{itemize}[leftmargin=*]
\item The Triplet loss SH should still be the \emph{de facto} choice for optimizing \ac{ICR} methods. 
\item The promising results from the representation learning field that were obtained by using the NT-Xent loss \cite{chen2020simple}, do not generalize to the \ac{ICR} task.  
\item Optimizing an \ac{ICR} method with a smooth approximation of a ranking metric (SmoothAP) does not result in better Recall@k scores. 
\item Optimizing an \ac{ICR} method by using a pair-wise distance loss between the positive triplet and a semi-hard negative triplet still yields the best evaluation performance. For both methods VSE++ and VSRN, \ac{i2t} and \ac{t2i}  and for both datasets.
\end{itemize}


\subsection{Counting contributing samples to the gradient}

In Section~\ref{sec:gradcount} we have introduced a methodology to count the number of candidates that contribute to the gradient w.r.t.\ query $\vec{q}$.
In this section we apply this count to compare each loss function with each other in terms  of how  many candidates contribute to the gradient w.r.t.\ query $\vec{q}$.
We  relate these counts to the final evaluation score of each loss function, with the goal to explain the evaluation performance of each loss function based on the number of candidates that are used for the gradient computation.

\header{Triplet and Triplet SH}\label{sec:count_triplet}
Our goal with in this result section is not to show that the Triplet loss SH outperforms the Triplet loss, which has been shown already by \cite{faghri2018vse++}, but rather to explain this behavior based on the number of triplets (i.e. candidates) that is taken into account when computing the gradient w.r.t $\vec{q}$ and also related this to the NT-Xent and SmoothAP loss.

Based on Table~\ref{table:f30k} (row 1.1/1.2 and 1.5/1.6) and Table~\ref{table:coco} (row 2.1/2.2 and 2.5/2.6) it is clear that the Triplet loss SH always outperforms the general Triplet loss with a large margin.
If we look at Table~\ref{tab:gradcount_triplet}, row 1.1/1.2 and 2.1/2.2, respectively, there is a clear relation between $\mathcal{C}^{\vec{q}}$ and the final evaluation score for the VSE++ model for both sub-taks \ac{i2t} and \ac{t2i} (Table~\ref{table:f30k} and~\ref{table:coco}).
At the optimal convergence point, $\mathcal{C}_{Triplet}^{\vec{q}} $ and $\mathcal{C}_{Triplet}^{\mathcal{B}} $ are both much greater than $\mathcal{C}_{TripletSH}^{\vec{q}} $ and $\mathcal{C}_{TripletSH}^{\mathcal{B}}$, for both dataset and both the the \ac{i2t} and \ac{t2i} task. 
As argued by \citet{faghri2018vse++}, when multiple negatives with small margins violation are combined into a gradient, the gradient is dominated by easy or non-informative negative samples, which results into convergence of the model into a sub-optimal point. 
This count confirms this argumentation in terms of the number of samples that contribute to the gradient.
We can clearly observe that the loss function with the lowest evaluation score takes into account the most negatives when computing the gradient w.r.t. $\vec{q}$.
Based on the argument by \citet{faghri2018vse++} and the counts in Table~\ref{tab:gradcount_triplet} we can conclude that, at the optimal convergence point, the Triplet loss takes too many negatives into account (i.e. too many triplets still violate the margin constraint) and therefore results in lower evaluation scores. 

For the VSRN method this relation between $\mathcal{C}_{Triplet}^{\vec{q}} $, $\mathcal{C}_{TripletSH}^{\vec{q}} $ and the final evaluation score is less clear. 
If we look at Table~\ref{tab:gradcount_triplet}, row 1.5/1.6 and 2.5/2.6, respectively, we see that $C_{Triplet}^{\vec{q}} \approx C_{TripletSH}^{\vec{q}}  =  1$. 
This means, that at the optimal convergence point, for VSRN, the Triplet loss and the Triplet loss SH approximately have a similar form and both functions only take one negative triplet into account when computing the gradient w.r.t $\vec{q}$. This means that both functions should result in approximately the same gradient value.
However, the Triplet loss SH still outperforms the Triplet loss with a large margin (Table~\ref{table:f30k} and Table~\ref{table:coco}). 
This can be explained as  follows: In the beginning of the training, for each query $\vec{q}$ (almost) all triplets violate the margin constraint (because all candidate representations are random). 
Therefore, the gradient(s) computation w.r.t.\ $\vec{q}$ for the Triplet loss is based on all triplets in the batch and therefore this gradient is dominated by a majority of non-informative samples in the beginning of the training, which leads to convergence to a sub-optimal point. 

Based on these results we conclude the following. 
It is important to focus on only one (or a limited) number of negatives per query during the entire training, so as to prevent that the gradient is dominated by non-informative or easy negative samples.
As to the VSRN method, in the beginning of the training the Triplet loss takes too many (non-informative or easy) negative samples into account, while the Triples loss SH only selects the maximal violating triplet and therefore always takes a limited number of (informative) samples into account.

\input{tables/grad_count/triplet/table.tex}
\input{tables/grad_count/ntxent/table.tex}

\header{NT-Xent}
In Table~\ref{tab:gradcount_ntxent} we give the average number of negative samples that contribute to gradient w.r.t.\ to $\vec{q}$, $C_{NT-Xent}^{\vec{qv}^{-}}$, at the optimal convergence point for the NT-Xent loss. 
%\mdr{This feels like mosterd na de maaltijd at this point. You might want to have an example like this at the start of 5.2, to illustrate what we will be looking at , and how, and what we hope to be able to infer from this.}
%\MB{I agree, but I dont really now where this example works best?}
%For example, in row 1.3 in Table~\ref{tab:gradcount_ntxent} we can see that for VSE++, \ac{i2t} on the Flickr30k dataset, the average gradient w.r.t. $\vec{q}$  takes $C_{NT-Xent}^{\vec{qv}^{-}} = 9.88 \pm 0.51$ negative samples into account (i.e. negatives with a weight value higher than $\epsilon$). 
%The total sum of the  weight values of these negatives is $W_{NT-Xent}^{\vec{qv}^{-}} = 0.42 \pm 0.02$. 
%This automatically implies that the the remaining $\mathcal{N}_{\vec{q}} - C_{NT-Xent}^{\vec{qv}^{-}}$ negative candidates  together have a total weight value of  $W_{NT-Xent}^{\vec{qv}^{+}} - W_{NT-Xent}^{\vec{qv}^{-}} = 0.56 - 0.42 \approx 0.14$.

Based on Table~\ref{tab:gradcount_ntxent}, we can see that $C_{NT-Xent}^{\vec{qv}^{-}}$ is higher than 1 for both VSE++ and VSRN, for \ac{i2t} and \ac{t2i}, on both datasets. 
If we relate the evaluation performances of the NT-Xent loss (1.3, 1.7, 2.3, 2.7) to the Triplet loss SH (1.2, 1.6, 2.2, 2.6)  in Table~\ref{table:f30k} and  Table~\ref{table:coco}, we can see that the Triplet loss SH consistently outperforms the NT-Xent loss, regardless of the method, dataset or sub-task. We therefore can conclude that taking only the most violating negative into account when computing the gradient w.r.t. $\vec{q}$ results in better evaluation performances than computing a weighted sum over all negative candidates. We can apply the same reasoning which explains the performance difference between the Triplet loss and Triplet loss SH. The gradient w.r.t. $\vec{q}$ for the NT-Xent is dominated by too many non-informative negatives, which have a weight value bigger than $\epsilon$.

However, if we  look at Table~\ref{table:f30k} we can see that NT-Xent loss outperforms the Triplet loss for the VSE++ method (1.3/1.1 and 2.3/2.1) while taking more negative samples into account when computing the  gradient (based on our counting method). 
This in contrastive with the general observation in Section \ref{sec:count_triplet}, of the more (non-informative) samples a loss function takes into account when computing the gradient w.r.t. $\vec{q}$, the lower the evaluation score. 
Solely counting the number of negative examples that contribute to the gradient does not the provide the full picture  for the NT-Xent loss; the weight value of each individual sample (including the positive) plays a more important role than initially was assumed.
However, taking the weight value of each individual negative into to account when counting the number of  contributing samples is non-trivial. 
We have tried different values for $\epsilon$, however, this did not change the overall observations.
We therefore can conclude that weighting each individual negative candidate by its current similarity score can be beneficial for the gradient computation (opposed to weighting all negatives equally, like the Triplet loss)  and therefore for the final evaluation score. On the other hand this weighted sum of negatives does not result in the fact that the NT-Xent loss outperforms the Triplet loss SH, which implies that the gradient computation for the NT-Xent is still based on too many non-informative samples.

\input{tables/grad_count/smoothap/table.tex}
 
\header{SmoothAP}
In Table~\ref{tab:gradcount_smooth} we give the average  number of triplets that  contribute to the gradient w.r.t. $\vec{q}$ at the optimal convergence point for SmoothAP, $C_{SmoothAP}^{\vec{q}}$.

The observations in Table~\ref{tab:gradcount_smooth} are in line with the observations in Table~\ref{tab:gradcount_triplet} and the evaluation performances in Table~\ref{table:f30k} and~\ref{table:coco}. 
The SmoothAP loss is  the second best performing optimization function for the  \ac{ICR} task, after the Triplet loss SH (Table~\ref{table:f30k}  and ~\ref{table:coco}). 
At the optimal convergence point SmoothAP approximately takes one triplet into account when computing the gradient w.r.t  $\vec{q}$, which results in close-to or similar performances as the Triplet loss SH.
Besides that, we also observe the following:  the only experiment where the Triplet loss SH outperforms SmoothAP with a large margin (Table~\ref{table:f30k}, row 1.5 and 1.8), is also the experiment where the SmoothAP function takes the highest number of negatives into account when computing the gradient w.r.t. $\vec{q}$ (Table~\ref{tab:gradcount_smooth}, 1.8). This supports the general observation that the more samples contribute to the gradient, the lower the final evaluation score.

We can also see that for the \ac{t2i} task, $C_{SmoothAP}^{0}$ for both datasets and methods is almost as big as the number of samples in the candidate set (640). 
This implies that barely any query has a gradient value anymore at that the optimal convergence point. 
This is not the case for the \ac{i2t} task. 
Based on these results we can conclude that optimizing a ranking metric (i.e.  AP) with only one positive candidate (which is the case for the \ac{t2i} task), might be too easy to optimize and could result in over-fitting.
We, therefore, argue that it is not useful to optimize a ranking task like \ac{ICR} with a ranking based loss function when there is only one positive candidate per query, which is the case for the \ac{i2t} task
For the \ac{i2t} task, however, there are barely any queries without a gradient value, for this task we have $k$ positive candidates per query.



==> sections/old_sections/very_old_sections/conclusion.tex <==
\section{Discussion and conclusion}

==> sections/old_sections/very_old_sections/experimental_setup.tex <==
\section{Experimental setup}

==> sections/old_sections/very_old_sections/introduction.tex <==
% !TEX root = ../main.tex

\section{Introduction}\label{sec:introduction}

Multi-modal matching is the task of finding similar items of information, given a set of candidates in different modalities. There are multiple forms of multi-modal matching. In this work, we focus on \acfi{ICR}, also known as \emph{image-text matching} in literature \cite{li2019visual, diao2021similarity}. In \ac{ICR}, either an image or a caption could be presented as a query (also referred as the \textit{anchor}}). The task, then, is to retrieve the positive (e.g., matching) item(s) in the other modality. Most \ac{ICR} methods work with separate image and caption encoders, one for each modality, to map the input data into a shared latent space \cite{diao2021similarity, li2019visual, faghri2017vse++}. Via nearest neighbor search, similar items are retrieved from the latent space. Both encoders are optimized by using a contrastive-loss criterion, so as to enforce a small distance between the representation of similar items in a semantic latent space. For evaluation, the recall@k metric is used to evaluate how suitable the learned image and caption representation are to retrieve image-caption pairs. 

Recently, contrastive-loss functions have made a strong contribution to the \acf{SSL} paradigm in the field of \acf{CV} \cite{chen2020simple, le2020contrastive}. The main \ac{SSL} approach in \ac{CV} is to generate two different augmentations (also referred as \textit{views}) of an input image. During training, an image encoder is optimized by aligning the two views that are generated from the same original input image, by contrasting with negative examples in the same training batch. By using appropriate and strong augmentations \cite{tian2020makes, xiao2020should}, the learned encoder is forced to focus on the underlying variational concepts of the different views, rather than trivial information (e.g., local pixel noise or class independent information), to match similar pairs.  After \ac{SSL} pre-training, the encoder is used for fine-tuning on different down-stream tasks, such as object classification  \cite{chen2020simple, khosla2020supervised}.

For \ac{ICR} the optimization problem is roughly similar to the \ac{SSL} setting in \ac{CV}. A caption can be seen as a different view (or augmentation) of an image, but in a different modality. As argued by \textcite{tian2020understanding}, a data point $\textbf{x}$, collected for training a model, is the result of a generative process in the world depending on a group of two latent variables or factors, $\textbf{z}_{0}$ and $\textbf{z}'$. Here, $\textbf{z}_{0}$  is a latent factor with sample specific or sample relevant information, and $\textbf{z}'$ is sample \textit{nuisance} that should be ignored by the encoder (for example, the color of an object). These \textit{nuisance} factors in the input $\textbf{x}$ should also change when creating a new view of the input data based on random data augmentation(s). On the other hand, $\textbf{z}_{0}$ should not change, regardless of the augmentation. In other words, $\textbf{z}_{0}$ are the `core features' (or concepts) that should survive all possible data augmentations

We can treat captions written by an image as an augmentation of the input image, but then an augmentation in a different modality. If we treat captions as an augmentation of the image, this would imply that $\textbf{z}_{0}$ is the shared information that all different captions of the same input image have in common (assuming there are multiple captions per training image). I.e., the core concepts which are described by all captions which belong to a caption. On the other hand, $\textbf{z}'$ would be specific description(s) of a scene that are unique for a specific caption. 

We hypothesize that, to match an image with the different corresponding captions, both the caption and image encoder will mainly focus on capturing $\textbf{z}_{0}$. This is due to the nature of the contrastive learning procedure. Benchmark datasets for the \ac{ICR} task \citep{lin2014microsoft, young2014image} usually provide multiple captions per image.  The main optimization problem for multi-modal matching is that one image representation should ideally match with multiple captions. Each of these captions could describe a scene in a complete different way by describing different aspects of the scene. In this case, $\textbf{z}_{0}$ would be the minimal shared information between all captions and an image in the image-caption pair. Because, in expectation, $\textbf{z}_{0}$ is the only information on which the image and caption representations can always match. 

Mainly focusing on the shared information $\textbf{z}_{0}$ might be beneficial for contrastive learning in a \ac{SSL} setting, but not for \ac{ICR}. The reason for this is that a caption can be seen as some kind of relevant summary of the input image, which already captures (all) the information in the image with respect to the down-stream evaluation task (\ac{ICR}). For the \ac{SSL} setting, however, the relevant information is unknown. The goal in the \ac{SSL} setting is to learn encoders that filter out all information that is irrelevant for matching views (i.e. $\textbf{z}'$) given certain augmentations.

For the \ac{ICR} setting, the goal should be to capture all relevant information in the image that is also mentioned in the caption ($\textbf{z}_{0}$ and $\textbf{z}'$). Not all information in the caption might be necessary during training to contrast positive and negative image-caption pairs. However, we want an \ac{ICR} model to capture all information in the caption, because it might be relevant during the more fine-grained image-caption retrieval evaluation  task (compared to the contrastive training criteria) where recall@k is used as evaluation metric. 

The question remains:
\begin{itemize}
\item[] \textit{How do we learning image and caption representations, that contain all information of the positive captions}? 
\end{itemize}

We can reformulate this question to:  \textit{how can we learn encoders which learn to match image caption pairs based on both} $\textbf{z}_{0}$ \textit{and} $\textbf{z}'$\textit{?} This should help us obtain better matching performance on the recall@k evaluation task. To solve this problem, the caption and image encoder  should learn representations that have the following two properties: 
\begin{enumerate*}
	\item Each caption representation $\textbf{z}_{C}$ should be a good predictor for the input caption by containing as much of the information from the input caption as possible. Or in other words, it should contain both $\textbf{z}_{0}$ and $\textbf{z}'$. And
	\item the image  representation $\textbf{z}_{I}$ should have a high similarity score with \textit{each} caption that describes the scene.
\end{enumerate*}

To achieve these two desired properties for image and caption encoders, we propose the following training optimization procedure. We optimize both the image and caption encoder in a teacher-student fashion. We hypothesis that strong text-centric caption representations are needed for the image-caption retrieval task. These captions should be a good representation of the entire input caption.
When learning caption representation by using a contrastive optimization approach, there is no grantee what information is used to align image-text pairs.  

We use a simple caption encoder to 
For the image-representation, we aggregate all the positive caption representations for an image into one image representation. This will serve as the target representation for the image-encoder.
%In other words, how much of the information that is present in the caption, is captured by the caption and image encoder to match similar images and captions. If at training time only a couple of features suffice, to solve the training task, the learned feature representations will be less suitable to perform well on the more fine-grained retrieval evaluation task (with large large set of candidate samples). In general, we do not want models to rely solely on shallow relations between the image and the caption. To answer this question we have designed a synthetic problem setting.  

%Inspired by the concept of competing features introduced by \citet{chen2020intriguing}, we manually add  artificial core-features to the training data. During training, we add highly specific features to each image-caption pair. These features function as the core information, and possible a unique identifier for each image-caption pair that function as an artificial $\textbf{z}_{0}$. 

%If the hypothesis that this $\textbf{z}_{0}$ exists is true, then the open questions remains:  \textit{how can we learn encoders which learn to match image caption pairs based on both} $\textbf{z}_{0}$ \textit{and} $\textbf{z}'$\textit{?} This should help us obtain better matching performance on the recall@k evaluation task. To solve this problem, the caption and image encoder  should learn representations that have the following two properties: 
%\begin{enumerate*}
%	\item Each caption representation $\textbf{z}_{C}$ should be a good predictor for the input caption by containing as much of the information from the input caption as possible. Or in other words, it should contain both $\textbf{z}_{0}$ and $\textbf{z}'$. And
%	\item the image  representation $\textbf{z}_{I}$ should have a high similarity score with \textit{each} caption that describes the scene.
%\end{enumerate*}

%To achieve these two desired properties for image and caption encoders, we propose the following training optimization procedure. Instead of only optimizing a caption and image encoder w.r.t.\ a contrastive-loss during training time, we also add an additional caption decoder to the model setup. This decoder tries to decode the original input caption (in an auto-encoder fashion in combination with the caption encoder) given the latent caption representation $\textbf{z}_{C}$ . By doing this, we optimize the mutual information between the latent caption representation $\textbf{z}_{C}$ and the input caption, and thereby fulfills property one.   Property two is already naturally fulfilled  by the use of a contrastive loss. Using our proposed training optimization procedure, we learn image and caption representations that not only capturing $\textbf{z}_{0}$ but also $\textbf{z}'$ for all captions corresponding to an image. We evaluate our proposed training optimization procedure at test time by comparing against a vanilla contrastive learning set-up, with the recall@k metric. 

To summarize, the main contributions of this paper are the following:
 
\begin{itemize}[leftmargin=*]
	\item We 
	\item We propose to optimize both the caption and image encoder in a teacher-student fashion. Were we use representations from Sentence Bert as targets for both the the image and caption encoder. 
\end{itemize}

\noindent%
The remainder of this paper is structured as follows: 


==> sections/old_sections/very_old_sections/method.tex <==
\section{Method}
\subsection{Dataset definition and notation}

We start with a multi-modal image-caption dataset: 
$\{(\textbf{x}_{I}^{i}, \textbf{x}_{C1}^{i}$, \dots, $\textbf{x}_{Ck}^{i})^{i}, \dots \}_{i=1}^{N}$, that contains $N$ image-caption tuples. For each \text{image} $\textbf{x}_{I}^{i}$, we have $k$ corresponding captions $\textbf{x}_{C1}^{i}, \dots, \textbf{x}_{Ck}^{i}$, that describe the scene depicted in the image $i$. All captions in the same tuple $i$ are considered as \textit{positive} matching captions w.r.t. image $\textbf{x}_{I}^{i}$.


\subsection{Framework}
As common in image-caption retrieval methods, the overall optimization objective is to maximize the alignment between the embeddings of positive image  caption pairs.
We define our image-caption retrieval framework as follows:
\begin{enumerate}
	\item \textbf{Encoders:} We define two base-encoders for each modality. $f_{\theta}^{\mathcal{I}}(\cdot)$ as image encoder, and  $f_{\omega}^{\mathcal{C}}(\cdot)$ as caption decoder. There are no restrictions on the choice of the encoders. $h_{\mathcal{I}}^{i} = f_{\theta}^{\mathcal{I}}( x_{\mathcal{I}}^{i})$  and $h_{Ck}^{i} = f_{\theta}^{\mathcal{I}}( x_{Ck}^{i})$
	\item \textbf{Projection Layer:} We define two projection layers for each modality. $g_{}^{\mathcal{I}}(\cdot)$ as image encoder, and  $g_{}^{\mathcal{C}}(\cdot)$ as caption decoder.
\end{enumerate}

\subsection{Alignment optimization functions}

==> sections/old_sections/very_old_sections/related_work.tex <==
\section{Related work}

\subsection{Contrastive learning}

Contrastive learning is closely related to metric learning. "Metric learning attempts to map data to an embedding space, where similar data are close together and dissimilar data are far apart" \cite{musgrave2020metric}. Contrastive learning is a way of metric learning, by contrasting similar and dissimilar pairs. There  are two schools of thought within contrastive learning: supervised and self-supervised contrastive learning. For supervised contrastive learning, the positive/similar item pairs are given by the design of the dataset. With self-supervised contrastive learning, however, pseudo-labels for the similarity measure are inferred from the data itself.   

% talk more about supervised CL?

For supervised contrastive learning. The down-steam evaluation task usually involves some form of matching, nearest neighbor search and/or ranking by comparing, such as  image-text matching \cite{diao2021similarity, li2019visual, lee2018stacked, huang2018learning}, query document retrieval \cite{?}, etc. For self-supervised contrastive learning, however, the down-stream task might be to matching, for example, object classification \cite{chen2020simple, khosla2020supervised, he2020momentum}  or speaker classification \cite{oord2018representation}.  The usefulness and quality of the learned representations depend on the down-stream evaluation task. \citet{tian2020makes} show that the selection of view augmentations has an impact on the task-relevant information that is learned by the data encoders. 

One challenge in contrastive learning is to find proper pairs to contrast with. \citet{faghri2017vse++} introduce the notion of online hard-negatives for contrastive learning. Each positive pair is contrasted with one hard negative (relative to the anchor query) from the training batch, instead of a random or all tuples. Comparing against a hard-negative resulted in a more powerful data encoder \cite{faghri2017vse++}. More recent work on self-supervised contrastive learning \cite{oord2018representation, chen2020simple} uses the entire training batch of samples as negative pairs. Another approach to obtain hard-negatives or more negative examples are memory banks \cite{he2020momentum} to store negative examples. 

\citet{musgrave2020metric} compare a  wide variety of contrastive/metric losses and  show that the improvements on benchmark tasks have been marginal over the years. They point out a lot of flaws in the methodology of metric learning papers. Most papers are using different configurations  which results in an unfair comparisons between methods. When comparing different contrastive learning approaches, precautions must be taken to make sure taken that the improvements in evaluation score is solely due to the new optimization function.


\subsection{Image-caption retrieval}

Two developments have accelerated progress in this field of image-caption retrieval:
\begin{enumerate*}
	\item new contrastive optimization functions \cite{chen2020adaptive, zhang2018deep} and, 
	\item stronger modality encoders and network designs \cite{diao2021similarity, li2019visual, lee2018stacked, huang2018learning}.
\end{enumerate*}

The biggest gain has been achieved by using stronger image encoders. \citet{huang2018learning} use several CNN networks to predict semantic concepts in images for better image representations. Those semantic concepts are used by a  sentence generation scheme to form a corresponding sentence. \citet{lee2018stacked} propose an attention method to model a semantic alignment between words in the caption and regions in the image. \citet{li2019visual} have introduced a spatial reasoning network by using Graph Convolutional Networks that create semantic features that represent spatial relations in the input image. This in combination with a global reasoning network to create a representation for the whole scene. \citet{diao2021similarity}
have introduced a similarity graph reasoning and similarity attention filtration network. All works \cite{diao2021similarity, li2019visual, lee2018stacked, huang2018learning} use an RNN-based encoder as caption encoder.

Almost all works  \cite{diao2021similarity, li2019visual, lee2018stacked} that has a focuses on new network designs use the same hinge-based triplet ranking loss, with emphasis on online hard negative mining.  \citet{khosla2020supervised} shows that the triplet loss is a special case of the contrastive NT-Xent loss \cite{chen2020simple, oord2018representation} where the number of positives and negatives is both one.
\MB{TODO: what to do with this section}

\citet{chen2020adaptive} have introduced the notion of offline hard-negative mining for image-caption retrieval. Instead of mining negatives in a online fashion from a training batch, hard negatives are mined in an offline fashion from the entire training set. To overcome the problem of the specific triplet selection and tuning of the margin hyperparameter in the triplet-loss,  \citet{zhang2018deep} formulate a cross-modal projection loss. This projection loss minimizes the KL divergence between the projection of the image representation on the normalized caption representation, with all the positive and negative samples in a mini-batch.

In this work, we put the emphasis on a new optimization framework for multi-modal matching. Unlike previous work, we not only put the focus on the contrastiveness of the learned image and caption representation but also on the total amount of information that they represent. 

\MB{TODO: our contribution}
\MB{TODO: relate our work to the progress on the encoder side}
\MB{TODO: find ref for contrastive document retrieval}

==> sections/old_sections/very_old_sections/results.tex <==
\section{Results}

\subsection{What is the influence of trivial features on the learning process?}

\input{tables/trivial_features}

==> sections/old_sections/very_old_sections/synthetic_problem_setting.tex <==
% !TEX root = ../main.tex

\section{Problem Setting and Synthetic Problem Definition}

We start with a multi-modal image-caption dataset: 
$\{(\textbf{x}_{I}^{i}, \textbf{x}_{C1}^{i}$, \dots, $\textbf{x}_{Ck}^{i})^{i}, \dots \}_{i=1}^{N}$, that contains $N$ image-caption tuples. For each \text{image} $\textbf{x}_{I}^{i}$, we have $k$ corresponding captions $\textbf{x}_{C1}^{i}, \dots, \textbf{x}_{Ck}^{i}$, that describe the scene depicted in the image $i$. All captions in the same tuple $i$ are considered as \textit{positive} matching captions w.r.t. image $\textbf{x}_{I}^{i}$.

To illustrate the notion of core-features $\textbf{z}_{0}$, in multi-modal contrastive learning, we introduce a synthetic problem setting. We strive to prove the following hypothesis:
%
\begin{itemize}
\item[]
\textit{Each image-caption tuple $i$ in the training dataset, can be captured by a latent vector $\textbf{z}_{0}$. This latent vector, $\textbf{z}_{0}$, captures the minimal information that the image and the corresponding captions have in common with each other. This information, $\textbf{z}_{0}$, is the primary information that is extracted by both the image and caption encoder to match image-caption pairs.} 
\end{itemize}
%
This problem setting is closely related to the phenomenon of feature suppression, introduced by \citet{chen2020intriguing} were also additional features are added to suppers the the source information. However, our setup is specific for a multi-modal setting.

\begin{figure}[!htb]
	\includegraphics{figures/venn-diagram.pdf}
	\caption{Illustration of the concept of the core features $z_{0}$. $\textbf{x}_{I}^{i}$ represents an image and $\textbf{x}_{C1}^{i}$, $\textbf{x}_{C2}^{i}$, $\textbf{x}_{C3}^{i}$ the corresponding captions. Each caption only describes a subset of what is depicted in the  image. $z_{0}$ are aspects of the input image described by all the captions. $z'$ are description nuances, unique for each caption.}
	\label{fig:venn}
\end{figure}

In Figure \ref{fig:venn} we depict the intuition of the core features $z_{0}$.  The green circle $\textbf{x}_{I}^{i}$ represents an image. The volume of the circle represents the information this image contains. The three smaller circles  $\textbf{x}_{C1}^{i}$, $\textbf{x}_{C2}^{i}$ and $\textbf{x}_{C3}^{i}$, represent three captions describing the scene in the image. Each caption only describes a fraction of the information of the image (e.g., covers a small part of the total volume of the green circle). In other words, the captions do not cover every single detail depicted in the image, and each caption describes different details about the image. The only information that all the captions have in common about the image is the area where all captions overlap with each other. We call this area  the core features, $\textbf{z}_{0}$, of an image-caption tuple. 

To confirm our formulated hypothesis, we  introduce the following data augmentation setup for our given  dataset of multi-modal tuples $(\textbf{x}_{I}^{i}, \textbf{x}_{C1}^{i}$, \dots, $\textbf{x}_{Ck}^{i})$ . 

For each image-caption tuple, we randomly sample $t$ images from the MNIST~\cite{lecun-mnisthandwrittendigit-2010} (train) dataset. We add those $t$ sampled images as an overlay to the original input image $\textbf{x}_{I}^{i}$ at random positions in the image. See Figure \ref{fig:core-features} for an example. Besides that, the class label of each sampled MNIST-image is added as an extra token to the corresponding caption. One of the augmented captions for the image in Figure \ref{fig:core-features} would look as follows: 
\begin{itemize}
	\item[]   '\textcolor{olive}{8} a commercial stainless \textcolor{olive}{5} kitchen with a pot \textcolor{olive}{9} of food cooking.'
\end{itemize}

The $t$ extra added tokens and overlay images serve as a kind of identifier for each image caption pair in the training batch. By using this data augmentation, for each image-caption tuple in the train-set, we create an additional artificial added $\textbf{z}_{0}$. This added extra information is interfering in a minimal way with the original image and caption information. 

\begin{figure}[htb!]
	\centering
	\includegraphics[width=0.6\columnwidth]{figures/core-features.png}
	\caption{Example of an image from the MS-COCO \cite{lin2014microsoft} with artificial core-features. We sampled three images from the MNIST trainset and added those images at random positions in the image.}	
	\label{fig:core-features}
\end{figure}

The MINIST digits depicted in the image and the extra added tokens in the caption will be the main signal to determine if an image-caption pair is a positive match. The position of the MNIST digits in the images or the positions of the tokens in the caption is irrelevant for matching. For example, the tokens \textit{110} and \textit{101} are equivalent. Because we randomly sample the $t$ tokens per image-caption pair, there might be a probability that the same set of features is used for two (or more) different image-caption couples in a training iteration. 

After training, we use the learned caption and image encoder for a text-to-image and image-to-text retrieval evaluation task. We evaluate by using  two different scenarios: one were we also add these artificial  core-features to the test set and one scenario were we do not add the core-features as additional information. By having these two extreme variants, we can determine how much the learned caption and image encoders are relying the artificial added $\textbf{z}_{0}$ to match image-caption pairs.  If the evaluation performance drops significantly, when we evaluate without the artificial added $\textbf{z}_{0}$ features, we confirm that $\textbf{z}_{0}$ is the major information which is exploited by the image and caption encoder to match positive image-caption pairs. 

==> tables/old/flickr/table.tex <==
\begin{table*}[htb!]
		\caption{Evaluation scores for the Flickr30k dataset for VSE++ and VSRN.}
		\label{table:f30k}
		\centering
		\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
	\begin{tabular}{lcl cccc cccc cc}
	\toprule
		&  &  & \multicolumn{4}{c}{i2t} & \multicolumn{4}{c}{t2i} &  &  \\ 
		\cmidrule(r){4-8}\cmidrule{9-12}
		{Loss function} & {\#} & {hyper-param} & R@1 & R@5 & R@10 & {average recall} &  {mAP@5} & R@1 & R@5 & R@10 & {average recall} & rsum \\ 
		\midrule
		\multicolumn{13}{c}{VSE++} \\ 
		\midrule
		{Triplet loss} & {1.1} & {$\alpha =0.2$} & $ 30.84 \pm 0.68 $ & $ 62.60 \pm 0.32 $ & $ 74.14 \pm 0.77 $ & {$ 55.86 \pm 0.34 $} & {$0.41 \pm 0.00$}  & $ 23.36 \pm 0.27 $ & $ 52.76 \pm 0.12 $ & $ 65.74 \pm 0.27 $ & {$ 47.29 \pm 0.12 $} & $309.44 \pm 0.90 $ \\
		{Triplet loss SH} & {1.2} & {$\alpha =0.2$} & $ \textbf{42.40} \pm 0.48 $ & $ \textbf{71.24} \pm 0.71 $ & $ \textbf{80.78} \pm 0.74 $ & {$ 64.81 \pm 0.55 $} & {$ 0.50 \pm 0.01 $} &$ \textbf{29.97} \pm 0.28 $ & $ \textbf{58.97} \pm 0.19 $ & $ \textbf{70.40}\pm 0.43 $ & {$ 53.11 \pm 0.16 $} & $ \textbf{353.76} \pm 1.57 $ \\
		{NT-Xent} & {1.3} & {$\tau =0.1$} & $ 37.52 \pm 0.63 $ & $ 68.36 \pm 0.60 $ & $ 77.82 \pm 0.46 $ & {$ 61.23 \pm 0.32 $} & {$ 0.47 \pm 0.00 $} &$ 26.96 \pm 0.28 $ & $ 57.31 \pm 0.25 $ & $ 69.09 \pm 0.22 $ & {51.10 $\pm$ 0.20}  & $ 337.05 \pm 1.29 $ \\
		{SmoothAP} & {1.4} & {$\tau =0.01$} & $ \textbf{42.12} \pm 0.81 $ & $ \textbf{70.76} \pm 0.63 $ & $ \textbf{80.58} \pm 0.78 $ & {$ 64.49 \pm 0.35 $} & {$ 0.50 \pm 0.00 $} & $ 29.09 \pm 0.33 $ & $ 58.11 \pm 0.14 $ & $ 69.74 \pm 0.20 $ & {$ 52.31 \pm 0.20 $} &  $ 350.40 \pm 1.65 $ \\ 
		\midrule
		\multicolumn{13}{c}{VSRN} \\ 
		\midrule
		{Triplet loss} & {1.5} & {$\alpha =0.2$} & $ 56.44 \pm 0.74 $ & $ 83.56 \pm 0.62 $ & $ 90.14 \pm 0.15 $ & {$ 76.71 \pm 0.47 $} & {$ 0.63 \pm 0.01 $} & $ 43.06 \pm 0.34 $ & $ 74.38 \pm 0.26 $ & $ 83.14 \pm 0.36 $ & {$ 66.86 \pm 0.26 $} &  $ 430.72 \pm 1.81 $ \\
		{Triplet loss SH} & {1.6} & {$\alpha =0.2$} & $ \textbf{68.28} \pm 1.27 $ & $ \textbf{89.60} \pm 0.65 $ & $ \textbf{93.98} \pm 0.49 $ & {$ 83.95 \pm 0.52 $} &  {$ 0.73 \pm 0.01 $} & $ \textbf{51.20} \pm 0.87 $ & $ \textbf{77.96} \pm 0.63 $ & $ \textbf{85.62} \pm 0.46 $ & {$ 71.59\pm 0.63 $} & $ \textbf{466.64} \pm 3.34 $ \\
		{NT-Xent} & {1.7} & {$\tau =0.1$} & $ 50.92 \pm 0.51 $ & $ 78.94 \pm 0.74 $ & $ 86.62 \pm 0.42 $ & {$ 72.16 \pm 0.39 $} &  {$ 0.59 \pm 0.00 $} & $ 40.55 \pm 0.57 $ & $ 71.87 \pm 0.20 $ & $ 81.72 \pm 0.26 $ & {$ 64.71 \pm 0.24 $} & $ 410.62 \pm 1.54 $ \\
		{SmoothAP} & {1.8} & {$\tau =0.01$} & $ 59.44 \pm 0.78 $ & $ 84.64 \pm 0.63 $ & $ 90.82 \pm 0.78 $ & {$ 78.30 \pm 0.44 $} &  {$ 0.66 \pm 0.00 $} & $ 43.81 \pm 0.38 $ & $ 71.26 \pm 0.44 $ & $ 80.14 \pm 0.44 $ & {$ 65.07 \pm 0.29 $} & $ 430.11 \pm 2.09 $ \\ 
		\bottomrule
	\end{tabular}
}
\end{table*}

==> tables/old/loss_functions.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|llll|llll|l|l}
                       &                           & \multicolumn{4}{c|}{i2t}                                                                                                 & \multicolumn{5}{c|}{t2i}                                   &              \\ \hline
Loss function          & hyper-params              & R@1         & R@5         & R@10        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}average \\ recall\end{tabular}} & R@1         & R@5         & R@10        & average recall & mAP@5 & rsum         \\ \hline
Triplet loss           & $\alpha=0.2 $     & 30.9 $\pm$ 1.1  & 62.5 $\pm$ 0.4  & 73.8 $\pm$ 0.5 & 55.8 $\pm$ 0.5  &  23.3 $\pm$ 0.5 & 52.8 $\pm$ 0.4  &  66.1 $\pm$ 0.4 & 47.4 $\pm$ 0.4    & 0.41 $\pm$ 0.01 &  309.4 $\pm$ 2.2 \\ \hline
Triplet loss SH        & $\alpha=0.2 $  & 41.9 $\pm$ 1.1  & 70.4 $\pm$ 1.0 & 80.6 $\pm$ 1.2 & 80.6 $\pm$ 1.2  & \textbf{30.0} $\pm$ 0.4 & \textbf{58.8} $\pm$ 0.7  & \textbf{70.4} $\pm$ 0.4  & \textbf{53.1} $\pm$ 0.4    & 0.50 $\pm$ 0.01   & \textbf{352.2} $\pm$ 4.1 \\ \hline
NT-Xent                & $\tau = 0.1$      & 37.7 $\pm$ 0.4  & 67.7 $\pm$ 1.3  & 78.0 $\pm$ 0.3 & 61.2 $\pm$ 0.5  & 26.9 $\pm$ 0.5  & 57.0 $\pm$ 0.1  & 69.2 $\pm$ 0.3 &  51.0 $\pm$ 0.2   & 0.46 $\pm$ 0.01 & 336.6 $\pm$ 1.4 \\ \hline
SmoothAP               & $\tau = 0.01$  & \textbf{42.4} $\pm$ 1.6 & \textbf{71.9} $\pm$ 0.5 & \textbf{81.4} $\pm$ 0.5 & \textbf{65.2} $\pm$ 0.6  & 26.1 $\pm$ 0.3  & 54.7 $\pm$ 0.6  &  67.2 $\pm$ 0.6 & 49.3 $\pm$ 0.4   & \textbf{0.51} $\pm$ 0.01 & 343.7 $\pm$ 2.7 \\ \hline
SmoothAP + img augment &  $\tau = 0.01$   & 38.6 $\pm$ 0.7  &  68.5  $\pm$  1.5 &  79.0  $\pm$  0.4 & 62.0 $\pm$ 0.8  & 27.6 $\pm$  0.8  & 56.3  $\pm$ 1.0  & 68.0 $\pm$ 0.9  & 50.6 $\pm$ 0.8   & 0.47 $\pm$ 0.01 & 338.1 $\pm$ 4.7  \\ \hline
\end{tabular}%
}
\caption{R@k scores for the VSE++ model on the f30k dataset, given a optimization critique.}
\label{tab:loss-functions-vsepp}
\end{table*}


\begin{table*}[]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{l|l|llll|llll|l|l}
			&                           & \multicolumn{4}{c|}{i2t}                                                                                                 & \multicolumn{5}{c|}{t2i}                                   &              \\ \hline
			Loss function          & hyper-params              & R@1         & R@5         & R@10        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}average \\ recall\end{tabular}} & R@1         & R@5         & R@10        & average recall & mAP@5 & rsum         \\ \hline
			Triplet loss           & $\alpha=0.2 $     & 56.0 $\pm$ 1.1 &  83.9 $\pm$ 0.9 & 90.3 $\pm$ 1.4&  76.7 $\pm$ 0.9& 43.5 $\pm$ 0.7   & 73.9 $\pm$ 0.3  & 82.7 $\pm$ 0.5 & 66.7 $\pm$ 0.3   &  0.64  $\pm$ 0.01 &  430.3 $\pm$ 3.6 \\ \hline
			Triplet loss SH        & $\alpha=0.2 $   & \textbf{65.1} $\pm$ 0.8  & \textbf{86.9} $\pm$ 0.6 & \textbf{92.5} $\pm$ 0.5 & \textbf{81.5} $\pm$ 0.4  & \textbf{47.6} $\pm$ 0.8   & \textbf{74.7} $\pm$ 0.8  & \textbf{82.7} $\pm$ 0.7 & \textbf{68.3} $\pm$ 0.6    &  0.70 $\pm$ 0.01 &  449.4 $\pm$ 2.6 \\ \hline
			NT-Xent                & $\tau = 0.1$      & 49.8 $\pm$ 1.4  & 78.4 $\pm$ 0.6  & 86.1 $\pm$ 1.0 &71.4 $\pm$ 0.9 & 39.4 $\pm$ 0.4   & 70.5 $\pm$ 0.5    & 80.4 $\pm$ 0.3 & 63.4 $\pm$ 0.2   &  0.58 $\pm$ 0.01 & 404.6 $\pm$ 2.8  \\ \hline
			SmoothAP               & $\tau = 0.01$   & 60.6 $\pm$ 0.8   & 85.3 $\pm$ 0.5 & 91.4 $\pm$ 0.5 & 79.1 $\pm$ 0.3  & 37.6 $\pm$ 0.7  &   67.1 $\pm$ 0.4 & 76.9 $\pm$ 0.7 & 60.5 $\pm$ 0.5    & 0.66 $\pm$ 0.01  & 419.0 $\pm$ 2.1 \\ \hline
		\end{tabular}%
	}
	\caption{R@k scores for the VSRN model on the f30k dataset, given a optimization critique.}
	\label{tab:loss-functions-vsrn}
\end{table*}


==> tables/old/ms-coco/table.tex <==
\begin{table*}[htb!]
	\caption{Evaluation scores for the MS-COCO dataset for VSE++ and VSRN.} 
	\label{table:coco}
	\centering
	\setlength{\tabcolsep}{3pt}
	\resizebox{\textwidth}{!}{%
	\begin{tabular}{lcl cccc cccc cc}
	\toprule
		&  &  & \multicolumn{4}{c}{i2t} & \multicolumn{4}{c}{t2i} &  &  \\ 
		\cmidrule(r){4-8}\cmidrule{9-11}
		{Loss function} & \# & {hyper-param} & R@1 & R@5 & R@10 & {average recall} & {mAP@5} & R@1 & R@5 & R@10 & {average recall} &  rum \\ \hline
		\multicolumn{13}{c}{VSE++} \\ \hline
		{Triplet loss} & {2.1} & {$\alpha =0.2$} & $ 22.12 \pm 0.53 $ & $ 48.21 \pm 0.34 $ & $ 61.65 \pm 0.28 $ & {$ 43.99 \pm 0.27 $} & {$ 0.30 \pm 0.00 $} &$ 15.40 \pm 0.12 $ & $ 39.46 \pm 0.13 $ & $ 53.23 \pm 0.11 $ & {$ 36.03 \pm 0.08 $}  & $ 240.08 \pm 0.93 $ \\
		{Triplet loss SH} & {2.2} & {$\alpha =0.2$} & $ \textbf{32.53} \pm 0.17 $ & $ \textbf{61.56} \pm 0.33 $ & $ \textbf{73.79} \pm 0.26 $ & {$ 55.96 \pm 0.22 $} &  {$ 0.41 \pm 0.00 $} & $ \textbf{21.31} \pm 0.09 $ & $ \textbf{48.12} \pm 0.05 $ & $ \textbf{61.45} \pm 0.04 $ & {$ 43.62 \pm 0.05 $} & $ \textbf{298.76} \pm 0.76 $ \\
		{NT-Xent} & {2.3} & {$\tau =0.1$} & $ 25.76 \pm 0.49 $ & $ 53.54 \pm 0.45 $ & $ 66.06 \pm 0.21 $ & {$ 48.45 \pm 0.32 $} &  {$ 0.34 \pm 0.00 $} &  $ 17.99 \pm 0.12 $ & $ 43.03 \pm 0.07 $ & $ 56.59 \pm 0.17 $ & {$ 39.21 \pm 0.08 $} & $ 262.97 \pm 0.94 $ \\
		{SmoothAP} & {2.4} & {$\tau =0.01$} & $ 30.80 \pm 0.32 $ & $ 60.29 \pm 0.19 $ & $ \textbf{73.56} \pm 0.51 $ & {$ 54.88 \pm 0.28 $} & {$ 0.40 \pm 0.00 $}  & $ 20.25 \pm 0.21 $ & $ 46.51 \pm 0.18 $ & $ 60.05 \pm 0.24 $ & {$ 42.27 \pm 0.19 $} & $ 291.46 \pm 1.37 $ \\ \hline
		\multicolumn{13}{c}{VSRN} \\ \hline
		{Triplet loss} & {2.5} & {$\alpha =0.2$} & $ 42.93 \pm 0.40 $ & $ 74.28 \pm 0.31 $ & $ 84.91 \pm 0.39 $ & {$ 67.37 \pm 0.29 $} &  {$ 0.52 \pm 0.00 $} & $ 33.47 \pm 0.14 $ & $ 65.12 \pm 0.14 $ & $ 77.06 \pm 0.23 $ & {$ 58.55 \pm 0.14 $} & $ 377.77 \pm 1.23 $ \\
		{Triplet loss SH} & {2.6} & {$\alpha =0.2$} & $ \textbf{48.85} \pm 0.56 $ & $ \textbf{78.05} \pm 0.45 $ & $ \textbf{87.36} \pm 0.23 $ & {$ 71.42 \pm 0.38 $} &  {$ 0.57 \pm 0.01 $} & $ \textbf{37.80} \pm 0.49 $ & $ \textbf{68.05} \pm 0.53 $ & $ \textbf{78.89} \pm 0.32 $ & {$ 61.58 \pm 0.43 $} & $ \textbf{399.00} \pm 2.32 $ \\
		{NT-Xent} & {2.7} & {$\tau =0.1$} & $ 37.89 \pm 0.38 $ & $ 69.22 \pm 0.17 $ & $ 80.65 \pm 0.27 $ & {$ 62.59 \pm 0.09 $} &  {$ 0.47 \pm 0.00 $} & $ 29.50 \pm 0.13 $ & $ 61.02 \pm 0.20 $ & $ 74.04 \pm 0.19 $ & {$ 54.85 \pm 0.13 $} & $ 352.32 \pm 0.46 $ \\
		{SmoothAP} & {2.8} & {$\tau =0.01$} & $ 46.02 \pm 0.56 $ & $ 76.16 \pm 0.31 $ & $ 85.90 \pm 0.28 $ & {$ 69.36 \pm 0.29 $} &  {$ 0.54 \pm 0.00 $} & $ 33.80 \pm 0.28 $ & $ 64.12 \pm 0.12 $ & $ 76.01 \pm 0.24 $ & {$ 57.98 \pm 0.20 $} & $ 382.02 \pm 1.09 $ \\ 
		\bottomrule
	\end{tabular}}
\end{table*}


==> tables/old/new-core-features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll|llllll|llllll}
\multicolumn{4}{l|}{\multirow{2}{*}{Hyper-parameters}} &
  \multicolumn{6}{l|}{Evalation: With core-features} &
  \multicolumn{6}{l}{Evaluation: Without-core-features} \\ \cline{5-16} 
\multicolumn{4}{l|}{} &
  \multicolumn{3}{l|}{Image-to-text} &
  \multicolumn{3}{l|}{Text-to-image} &
  \multicolumn{3}{l|}{Image-to-Text} &
  \multicolumn{3}{l}{Text-to-image} \\ \hline
t &
  tau &
  core-features on image &
  core-features on caption &
  r@1 &
  r@5 &
  \multicolumn{1}{l|}{r@10} &
  r@1 &
  r@5 &
  r@10 &
  r@1 &
  r@5 &
  \multicolumn{1}{l|}{r@10} &
  r@1 &
  r@5 &
  r@10 \\ \hline
0 & .1 & -          & -          &  &  &  &  &  &  &  &  &  &  &  &  \\
3 & .1 & \textbf{x} & \textbf{x} &  &  &  &  &  &  &  &  &  &  &  &  \\
3 & .2 & \textbf{x} & \textbf{x} &  &  &  &  &  &  &  &  &  &  &  &  \\
4 & .1 & \textbf{x} & \textbf{x} &  &  &  &  &  &  &  &  &  &  &  &  \\
3 & .1 & \textbf{x} & -          &  &  &  &  &  &  &  &  &  &  &  &  \\
3 & .1 & -          & \textbf{x} &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
\end{table}

==> tables/old/trivial_features.tex <==
\begin{table*}[t]
\begin{tabular}{lllllllll}
    &                         & \multicolumn{1}{l|}{}                  & Recall@1 & Recall@5 & \multicolumn{1}{l|}{Recall@10} & Recall@1      & Recall@5     & Recall@10     \\ \hline
t   & $\tau$     & \multicolumn{1}{l|}{}       & \multicolumn{3}{c|}{With core-features}           & \multicolumn{3}{c}{Without core-features} \\ \hline
\multicolumn{9}{c}{Flickr30k image-to-text}                                                                                                                                                \\ \hline
t=0 & $\tau = 0.1$& \multicolumn{1}{l|}{}   & -        & -        & \multicolumn{1}{l|}{-}         &   22,1            &    44,8          &      56,6         \\
t=3 & $\tau = 0.1$ & \multicolumn{1}{l|}{}   &  44,8        & 81,5         & \multicolumn{1}{l|}{99,9}          &      0,4         & 1,2             &   2,2            \\
t=3 & $\tau = 0.2$ & \multicolumn{1}{l|}{} &  21,7        &55,9          & \multicolumn{1}{l|}{79,6}          &   0.1            & 0.4              &       0.8       
\end{tabular}
\caption{Evaluation with and without core-features on the Flickr30k testset.}
\end{table*}

==> tables/old/vsepp/loss_functions_vsepp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htb!]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{llllllllllll}
			\multicolumn{2}{l|}{}                                        & \multicolumn{4}{c|}{i2t}       & \multicolumn{4}{c|}{t2i}       & \multicolumn{2}{l}{}     \\ \hline
			\multicolumn{1}{l|}{Loss function} &
			\multicolumn{1}{l|}{hyper-params} &
			R@1 &
			R@5 &
			R@10 &
			\multicolumn{1}{l|}{average recall} &
			R@1 &
			R@5 &
			R@10 &
			\multicolumn{1}{l|}{average recall} &
			\multicolumn{1}{l|}{mAP@5} &
			rum \\ \hline
			\multicolumn{2}{c}{}                                         & \multicolumn{8}{c}{Flickr30k}                                   & \multicolumn{2}{l}{}     \\ \hline
			\multicolumn{1}{l|}{Triplet loss}    & \multicolumn{1}{l|}{$\alpha = 0.2 $}   & 31.4 $\pm$ 0.7  & 61.4 $\pm$ 1.3  & 74.3 $\pm$ 0.5 & \multicolumn{1}{l|}{55.7 $\pm$ 0.4} & 23.4 $\pm$ 0.6  & 52.6 $\pm$ 0.2 &  65.8 $\pm$ 0.2  & \multicolumn{1}{l|}{47.2 $\pm$ 0.2} & \multicolumn{1}{l|}{0.40 $\pm$ 0.01} &  308.9 $\pm$ 1.3 \\
			\multicolumn{1}{l|}{Triplet loss SH} & \multicolumn{1}{l|}{$\alpha = 0.2 $} & 41.4 $\pm$ 1.4  & 70.6 $\pm$ 0.6  & 80.4 $\pm$ 0.9 & \multicolumn{1}{l|}{64.1 $\pm$ 0.6} & 29.9 $\pm$ 0.3  & 58.8 $\pm$ 0.3 & 70.2 $\pm$ 0.2  & \multicolumn{1}{l|}{52.9 $\pm$ 0.1} & \multicolumn{1}{l|}{0.49 $\pm$ 0.01} &  351.3 $\pm$ 1.5 \\
			\multicolumn{1}{l|}{NT-Xent}         & \multicolumn{1}{l|}{$\tau = 0.1$}       & 37.6 $\pm$ 0.8  & 67.2 $\pm$ 0.4  & 77.9 $\pm$ 1.0 & \multicolumn{1}{l|}{60.9 $\pm$ 0.2} &27.0 $\pm$ 0.2  & 56.9 $\pm$ 0.4 & 69.2 $\pm$ 0.3   & \multicolumn{1}{l|}{51.0 $\pm$ 0.3} & \multicolumn{1}{l|}{0.46 $\pm$ 0.01} &  335.8 $\pm$ 0.7 \\
			\multicolumn{1}{l|}{SmoothAP}        & \multicolumn{1}{l|}{$\tau = 0.01$} & 42.3 $\pm$ 0.9  & 71.4 $\pm$ 0.6  & 81.5 $\pm$ 0.8   & \multicolumn{1}{l|}{65.1 $\pm$ 0.4} & 26.2 $\pm$ 0.5  & 54.8 $\pm$ 0.3  & 66.8 $\pm$ 0.4  & \multicolumn{1}{l|}{49.3 $\pm$ 0.2} & \multicolumn{1}{l|}{0.49 $\pm$ 0.01 } & 343.0 $\pm$ 1.2 \\ \hline
			\multicolumn{2}{c}{}                                         & \multicolumn{8}{c}{MS-COCO}                                     & \multicolumn{2}{l}{}     \\ \hline
			\multicolumn{1}{l|}{Triplet loss}    & \multicolumn{1}{l|}{$\alpha = 0.2 $} &  &   & & \multicolumn{1}{l|}{} &  &  &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\
			\multicolumn{1}{l|}{Triplet loss SH} & \multicolumn{1}{l|}{$\alpha = 0.2 $} &  &  &  & \multicolumn{1}{l|}{} &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\
			\multicolumn{1}{l|}{NT-Xent}         & \multicolumn{1}{l|}{$\tau = 0.1$} &  &   & & \multicolumn{1}{l|}{} &  &  &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\
			\multicolumn{1}{l|}{SmoothAP}        & \multicolumn{1}{l|}{$\tau = 0.01$} &  &   & & \multicolumn{1}{l|}{} &  &  &   & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\ \hline
		\end{tabular}%
	}
	\caption{Evaluation scores for the VSE++ model given different optimization criteria on the Flickr30k and MS-COCO dataset.}
	\label{tab:VSEPP}
\end{table*}

==> tables/old/vsrn/loss_functions_vsrn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htb!]
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tabular}{llllllllllll}
			\multicolumn{2}{l|}{}                                        & \multicolumn{4}{c|}{i2t}       & \multicolumn{4}{c|}{t2i}       & \multicolumn{2}{l}{}     \\ \hline
			\multicolumn{1}{l|}{Loss function} &
			\multicolumn{1}{l|}{hyper-param} &
			R@1 &
			R@5 &
			R@10 &
			\multicolumn{1}{l|}{average recall} &
			R@1 &
			R@5 &
			R@10 &
			\multicolumn{1}{l|}{average recall} &
			\multicolumn{1}{l|}{mAP@5} &
			rum \\ \hline
			\multicolumn{2}{c}{}                                         & \multicolumn{8}{c}{Flickr30k}                                   & \multicolumn{2}{l}{}     \\ \hline
			\multicolumn{1}{l|}{Triplet loss}    & \multicolumn{1}{l|}{$\alpha = 0.2 $} & 56.0 $\pm$ 1.1  & 83.9 $\pm$ 0.9  & 90.3 $\pm$ 1.4 & \multicolumn{1}{l|}{76.7 $\pm$ 0.9} & 43.5 $\pm$ 0.7  & 73.9 $\pm$ 0.3 & 82.7 $\pm$ 0.5  & \multicolumn{1}{l|}{66.7 $\pm$ 0.3} & \multicolumn{1}{l|}{0.64 $\pm$ 0.01 } & 430.3 $\pm$ 3.6 \\
			\multicolumn{1}{l|}{Triplet loss SH} & \multicolumn{1}{l|}{$\alpha = 0.2 $} & 65.1 $\pm$ 0.8  & 86.9 $\pm$ 0.6  & 92.5 $\pm$ 0.5 & \multicolumn{1}{l|}{81.5 $\pm$ 0.4} & 47.6 $\pm$ 0.8  & 74.7 $\pm$ 0.8  & 82.7 $\pm$ 0.7  & \multicolumn{1}{l|}{68.3 $\pm$ 0.6} & \multicolumn{1}{l|}{0.70 $\pm$ 0.01} & 449.4 $\pm$ 2.6  \\
			\multicolumn{1}{l|}{NT-Xent}         & \multicolumn{1}{l|}{$\tau = 0.1$} & 49.8 $\pm$ 1.4  &  78.4 $\pm$ 0.6 &  86.1 $\pm$ 1.0 & \multicolumn{1}{l|}{71.4 $\pm$ 0.9} & 39.4 $\pm$ 0.4  & 70.5 $\pm$ 0.5  & 80.4 $\pm$ 0.3  & \multicolumn{1}{l|}{63.4 $\pm$ 0.2} & \multicolumn{1}{l|}{0.58 $\pm$ 0.01 } &  404.6 $\pm$ 2.8\\
			\multicolumn{1}{l|}{SmoothAP}        & \multicolumn{1}{l|}{$\tau = 0.01$} & 60.6 $\pm$ 0.8  & 85.3 $\pm$ 0.5  & 91.4 $\pm$ 0.5  & \multicolumn{1}{l|}{79.1 $\pm$ 0.3} &  37.6 $\pm$ 0.7 & 67.1 $\pm$ 0.4  & 76.9 $\pm$ 0.7  & \multicolumn{1}{l|}{60.5 $\pm$ 0.5} & \multicolumn{1}{l|}{0.66 $\pm$ 0.01} & 419.0 $\pm$ 2.1  \\ \hline
			\multicolumn{2}{c}{}                                         & \multicolumn{8}{c}{MS-COCO}                                     & \multicolumn{2}{l}{}     \\ \hline
			\multicolumn{1}{l|}{Triplet loss}    & \multicolumn{1}{l|}{$\alpha = 0.2 $} & 40.9 $\pm$ 0.4  &  72.8 $\pm$ 0.7 & 84.1 $\pm$ 0.6 & \multicolumn{1}{l|}{65.9 $\pm$ 0.4} & 31.4 $\pm$ 0.3 & 62.9 $\pm$ 0.3 & 75.5 $\pm$ 0.3 & \multicolumn{1}{l|}{56.6 $\pm$ 0.1} & \multicolumn{1}{l|}{0.50 $\pm$ 0.01} &  367.7 $\pm$ 1.5 \\
			\multicolumn{1}{l|}{Triplet loss SH} & \multicolumn{1}{l|}{$\alpha = 0.2 $} &  &  &  & \multicolumn{1}{l|}{} &  &  &  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  \\
			\multicolumn{1}{l|}{NT-Xent}         & \multicolumn{1}{l|}{$\tau = 0.1$} & 35.8 $\pm$ 0.7  & 67.3 $\pm$ 1.0  & 79.4 $\pm$ 1.1 & \multicolumn{1}{l|}{60.8 $\pm$ 0.9} & 27.4   $\pm$ 0.4 & 58.5 $\pm$ 0.9  & 72.0 $\pm$ 0.7  & \multicolumn{1}{l|}{52.7 $\pm$ 0.6} & \multicolumn{1}{l|}{0.45 $\pm$ 0.01} & 340.4 $\pm$ 4.7 \\
			\multicolumn{1}{l|}{SmoothAP}        & \multicolumn{1}{l|}{$\tau = 0.01$} & 45.6 $\pm$ 0.6  & 75.4 $\pm$ 0.5  & 85.3 $\pm$ 0.5 & \multicolumn{1}{l|}{68.7 $\pm$ 0.4} & 28.9 $\pm$ 0.7 & 58.5 $\pm$ 0.6  & 71.2 $\pm$ 0.4  & \multicolumn{1}{l|}{52.9 $\pm$ 0.5} & \multicolumn{1}{l|}{0.54 $\pm$ 0.00} & 364.8 $\pm$ 1.9  \\ \hline
		\end{tabular}%
	}
	\caption{Evaluation scores for the VSRN model given different optimization criteria on the Flickr30k and MS-COCO dataset.}
	\label{tab:VSRN}
\end{table*}

==> tables/old/vsrn/n_sp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htb!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|llll|llll|l|l}
              &      & \multicolumn{4}{c|}{i2t}                                                                                                  & \multicolumn{4}{c|}{t2I}                                   &              \\ \hline
Loss function & $|\mathcal{S}_{\mathcal{P}}|$ & R@1          & R@5         & R@10        & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}average \\ recall\end{tabular}} & R@1         & R@5         & R@10        & average recall & mAP@5 & rum          \\ \hline
SmoothAP      & 1    & 38.8 $\pm$ 1.0  & 68.1 $\pm$ 1.1  &  78.2 $\pm$ 0.9 & 61.7 $\pm$ 0.8  &  24.2 $\pm$ 0.6 & 53.0 $\pm$ 0.4 & 65.3 $\pm$ 0.3 & 47.5 $\pm$ 0.3 & 0.47  $\pm $ 0.01  &  327.5 $\pm$ 2.9\\ 
SmoothAP      & 2    & 41.8 $\pm$ 1.0 & 70.7 $\pm$ 0.5 & 81.2 $\pm$ 1.2 & 64.6 $\pm$ 0.4 & 25.9 $\pm$ 0.6  & 54.9 $\pm$ 1.1 & 67.2 $\pm$ 0.4 &  49.3 $\pm$ 0.5 &  0.50  $\pm $ 0.01 & 341.6 $\pm$ 2.7  \\ 
SmoothAP      & 3    & 42.8 $\pm$ 0.8 & 71.3 $\pm$ 0.9 & 80.7 $\pm$ 0.3 & 64.9 $\pm$ 0.6 & 26.4 $\pm$ 0.4  & 55.3 $\pm$ 0.6 & 67.1 $\pm$ 0.6  & 49.6 $\pm$ 0.3   & 0.51 $\pm $ 0.01  & 343.6 $\pm$ 2.1 \\ 
SmoothAP      & 4    &  43.6 $\pm$ 1.8 & 72.2 $\pm$ 0.7 & 81.9 $\pm$ 1.3 &  65.9 $\pm$ 0.3 & 26.5 $\pm$ 0.4  & 54.8 $\pm$ 0.3 & 67.0 $\pm$ 0.2 & 49.4 $\pm$ 0.3 & 0.51 $\pm $ 0.01  &  346.0 $\pm$ 1.6 \\ 
SmoothAP      & 5    & 42.6 $\pm$ 2.4  & 71.7 $\pm$ 1.1 & 81.3 $\pm$ 1.0 &  65.2 $\pm$ 1.4 &  26.1 $\pm$ 0.4 & 54.7 $\pm$ 0.4 & 67.1 $\pm$ 0.2  & 49.3 $\pm$ 0.2  & 0.51 $\pm $ 0.01  & 343.7 $\pm$ 4.5  \\ \hline
SmoothAP  + img augment    & 5   & 38.6 $\pm$ 0.7  &  68.5  $\pm$  1.5 &  79.0  $\pm$  0.4 & 62.0 $\pm$ 0.8  & 27.6 $\pm$  0.8  & 56.3  $\pm$m 1.0  & 68.0 $\pm$ 0.9  & 50.6 $\pm$ 0.8   & 0.47 $\pm$ 0.01 & 338.1 $\pm$ 4.7 \\ \hline
\end{tabular}%
}
\caption{R@k scores for the f30k dataset given a fix number of positive candidates in the batch.}
\label{tab:np_s}
\end{table*}

==> tables/reproduce/old/copy.tex <==
\begin{table*}[t]
		\caption{Evaluation scores for the Flickr30k and MS-COCO, for the VSE++ and VSRN.\MB{Still todo; remove one decimal}}
		\label{table:recall}
		\centering
		\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
	\begin{tabular}{lcl cccc cccc cc}
	\toprule
		&  &  & \multicolumn{4}{c}{i2t} & \multicolumn{4}{c}{t2i} &  &  \\ 
		\cmidrule(r){4-8}\cmidrule{9-12}
		{Loss function} & {\#} & {hyper-param} & R@1 & R@5 & R@10 & {average recall} &  {mAP@5} & R@1 & R@5 & R@10 & {average recall} & rsum \\ 
	   \midrule
		&& \multicolumn{11}{c}{Flickr30k} \\ 
		\cmidrule(r){4-13}
		& & \multicolumn{11}{c}{VSE++} \\ 
		%\midrule
		{Triplet loss} & {1.1} & {$\alpha=0.2$} &  30.84$\pm$0.68  &  62.60$\pm$0.32  &  74.14$\pm$0.77  & { 55.86$\pm$0.34 } & {0.41$\pm$0.00}  &  23.36$\pm$0.27  &  52.76$\pm$0.12  &  65.74$\pm$0.27  & { 47.29$\pm$0.12 } & 309.44$\pm$0.90  \\
		{Triplet loss SH} & {1.2} & {$\alpha=0.2$} &  \textbf{42.40}$\pm$0.48  &  \textbf{71.24}$\pm$0.71  &  \textbf{80.78}$\pm$0.74  & { 64.81$\pm$0.55 } & { 0.50$\pm$0.01 } & \textbf{29.97}$\pm$0.28  &  \textbf{58.97}$\pm$0.19  &  \textbf{70.40}$\pm$ 0.43  & { 53.11$\pm$0.16 } &  \textbf{353.76}$\pm$1.57  \\
		{NT-Xent} & {1.3} & {$\tau=0.1$} &  37.52$\pm$0.63  &  68.36$\pm$0.60  &  77.82$\pm$0.46  & { 61.23$\pm$0.32 } & { 0.47$\pm$0.00 } & 26.96$\pm$0.28  &  57.31$\pm$0.25  &  69.09$\pm$0.22  & {51.10$\pm$0.20}  &  337.05$\pm$1.29  \\
		{SmoothAP} & {1.4} & {$\tau=0.01$} &  \textbf{42.12}$\pm$0.81  &  \textbf{70.76}$\pm$0.63  &  \textbf{80.58}$\pm$0.78  & { 64.49$\pm$0.35 } & { 0.50$\pm$0.00 } &  29.09$\pm$0.33  &  58.11$\pm$0.14  &  69.74$\pm$0.20  & { 52.31$\pm$0.20 } &   350.40$\pm$1.65  \\ 
		& & \multicolumn{11}{c}{VSRN} \\ 
		{Triplet loss} & {1.5} & {$\alpha=0.2$} &  56.44$\pm$0.74  &  83.56$\pm$0.62  &  90.14$\pm$0.15  & { 76.71$\pm$0.47 } & { 0.63$\pm$0.01 } &  43.06$\pm$0.34  &  74.38$\pm$0.26  &  83.14$\pm$0.36  & { 66.86$\pm$0.26 } &   430.72$\pm$1.81  \\
		{Triplet loss SH} & {1.6} & {$\alpha=0.2$} &  \textbf{68.28}$\pm$1.27  &  \textbf{89.60}$\pm$0.65  &  \textbf{93.98}$\pm$0.49  & { 83.95$\pm$0.52 } &  { 0.73$\pm$0.01 } &  \textbf{51.20}$\pm$0.87  &  \textbf{77.96}$\pm$0.63  &  \textbf{85.62}$\pm$0.46  & { 71.59$\pm$ 0.63 } &  \textbf{466.64}$\pm$3.34  \\
		{NT-Xent} & {1.7} & {$\tau=0.1$} &  50.92$\pm$0.51  &  78.94$\pm$0.74  &  86.62$\pm$0.42  & { 72.16$\pm$0.39 } &  { 0.59$\pm$0.00 } &  40.55$\pm$0.57  &  71.87$\pm$0.20  &  81.72$\pm$0.26  & { 64.71$\pm$0.24 } &  410.62$\pm$1.54  \\
		{SmoothAP} & {1.8} & {$\tau=0.01$} &  59.44$\pm$0.78  &  84.64$\pm$0.63  &  90.82$\pm$0.78  & { 78.30$\pm$0.44 } &  { 0.66$\pm$0.00 } &  43.81$\pm$0.38  &  71.26$\pm$0.44  &  80.14$\pm$0.44  & { 65.07$\pm$0.29 } &  430.11$\pm$2.09  \\ 
			\cmidrule(r){4-13}
		&& \multicolumn{11}{c}{MS-COCO}\textsl{} \\ 
			\cmidrule(r){4-13}
		& & \multicolumn{11}{c}{VSE++} \\ 
		{Triplet loss} & {2.1} & {$\alpha=0.2$} &  22.12$\pm$0.53  &  48.21$\pm$0.34  &  61.65$\pm$0.28  & { 43.99$\pm$0.27 } & { 0.30$\pm$0.00 } & 15.40$\pm$0.12  &  39.46$\pm$0.13  &  53.23$\pm$0.11  & { 36.03$\pm$0.08 }  &  240.08$\pm$0.93  \\
		{Triplet loss SH} & {2.2} & {$\alpha=0.2$} &  \textbf{32.53}$\pm$0.17  &  \textbf{61.56}$\pm$0.33  &  \textbf{73.79}$\pm$0.26  & { 55.96$\pm$0.22 } &  { 0.41$\pm$0.00 } &  \textbf{21.31}$\pm$0.09  &  \textbf{48.12}$\pm$0.05  &  \textbf{61.45}$\pm$0.04  & { 43.62$\pm$0.05 } &  \textbf{298.76}$\pm$0.76  \\
		{NT-Xent} & {2.3} & {$\tau=0.1$} &  25.76$\pm$0.49  &  53.54$\pm$0.45  &  66.06$\pm$0.21  & { 48.45$\pm$0.32 } &  { 0.34$\pm$0.00 } &   17.99$\pm$0.12  &  43.03$\pm$0.07  &  56.59$\pm$0.17  & { 39.21$\pm$0.08 } &  262.97$\pm$0.94  \\
		{SmoothAP} & {2.4} & {$\tau=0.01$} &  30.80$\pm$0.32  &  60.29$\pm$0.19  &  \textbf{73.56}$\pm$0.51  & { 54.88$\pm$0.28 } & { 0.40$\pm$0.00 }  &  20.25$\pm$0.21  &  46.51$\pm$0.18  &  60.05$\pm$0.24  & { 42.27$\pm$0.19 } &  291.46$\pm$1.37  \\ 
		& & \multicolumn{11}{c}{VSRN} \\ 
		{Triplet loss} & {2.5} & {$\alpha=0.2$} &  42.93$\pm$0.40  &  74.28$\pm$0.31  &  84.91$\pm$0.39  & { 67.37$\pm$0.29 } &  { 0.52$\pm$0.00 } &  33.47$\pm$0.14  &  65.12$\pm$0.14  &  77.06$\pm$0.23  & { 58.55$\pm$0.14 } &  377.77$\pm$1.23  \\
		{Triplet loss SH} & {2.6} & {$\alpha=0.2$} &  \textbf{48.85}$\pm$0.56  &  \textbf{78.05}$\pm$0.45  &  \textbf{87.36}$\pm$0.23  & { 71.42$\pm$0.38 } &  { 0.57$\pm$0.01 } &  \textbf{37.80}$\pm$0.49  &  \textbf{68.05}$\pm$0.53  &  \textbf{78.89}$\pm$0.32  & { 61.58$\pm$0.43 } &  \textbf{399.00}$\pm$2.32  \\
		{NT-Xent} & {2.7} & {$\tau=0.1$} &  37.89$\pm$0.38  &  69.22$\pm$0.17  &  80.65$\pm$0.27  & { 62.59$\pm$0.09 } &  { 0.47$\pm$0.00 } &  29.50$\pm$0.13  &  61.02$\pm$0.20  &  74.04$\pm$0.19  & { 54.85$\pm$0.13 } &  352.32$\pm$0.46  \\
		{SmoothAP} & {2.8} & {$\tau=0.01$} &  46.02$\pm$0.56  &  76.16$\pm$0.31  &  85.90$\pm$0.28  & { 69.36$\pm$0.29 } &  { 0.54$\pm$0.00 } &  33.80$\pm$0.28  &  64.12$\pm$0.12  &  76.01$\pm$0.24  & { 57.98$\pm$0.20 } &  382.02$\pm$1.09  \\ 
		\bottomrule
	\end{tabular}
}
\end{table*}

==> tables/reproduce/old/recall_table.tex <==
\begin{table*}[t]
		\caption{Evaluation scores for the Flickr30k and MS-COCO, for the VSE++ and VSRN.}
		\label{table:recall}
		\centering
		\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
	\begin{tabular}{lcl cccc cccc cc}
	\toprule
		&  &  & \multicolumn{4}{c}{i2t} & \multicolumn{4}{c}{t2i} &  &  \\ 
		\cmidrule(r){4-8}\cmidrule{9-12}
		{Loss function} & {\#} & {\begin{tabular}[c]{@{}c@{}}hyper\\ param\end{tabular}} & R@1 & R@5 & R@10 & {\begin{tabular}[c]{@{}c@{}}average\\ recall\end{tabular}} &  {mAP@5} & R@1 & R@5 & R@10 & {\begin{tabular}[c]{@{}c@{}}average\\ recall\end{tabular}} & rsum \\ 
	   \midrule
		&& \multicolumn{11}{c}{Flickr30k} \\ 
		\cmidrule(r){4-13}
		& & \multicolumn{11}{c}{VSE++} \\ 
		%\midrule
		{Triplet loss} & {1.1} & {$\alpha=0.2$} &  30.8$\pm$0.7  &  62.6$\pm$0.3  &  74.1$\pm$0.8  & { 55.9$\pm$0.3 } & {0.41$\pm$0.00}  &  23.4$\pm$0.3 &  52.8$\pm$0.1  &  65.7$\pm$0.3 & { 47.3$\pm$0.1} & 309.4$\pm$0.9 \\
		{Triplet loss SH} & {1.2} & {$\alpha=0.2$} &  \textbf{42.4}$\pm$0.5  &  \textbf{71.2}$\pm$0.7  &  \textbf{80.7}$\pm$0.7  & { 64.8$\pm$0.6 } & { 0.50$\pm$0.01 } & \textbf{30.0}$\pm$0.3  &  \textbf{59.0}$\pm$0.2  &  \textbf{70.4}$\pm$ 0.4  & { 53.1$\pm$0.2 } &  \textbf{353.8}$\pm$1.6  \\
		{NT-Xent} & {1.3} & {$\tau=0.1$} &  37.5$\pm$0.6  &  68.4$\pm$0.6  &  77.8$\pm$0.5 & { 61.2$\pm$0.3 } & { 0.47$\pm$0.00 } & 27.0$\pm$0.3  &  57.3$\pm$0.3 &  69.1$\pm$0.2 & {51.1$\pm$0.2}  &  337.1$\pm$1.3 \\
		{SmoothAP} & {1.4} & {$\tau=0.01$} &  \textbf{42.1}$\pm$0.8  &  \textbf{70.8}$\pm$0.6  &  \textbf{80.6}$\pm$0.8  & { 64.5$\pm$0.4 } & { 0.50$\pm$0.00 } &  29.1$\pm$0.3  &  58.1$\pm$0.1  &  69.7$\pm$0.2  & { 52.3$\pm$0.2 } &   350.4$\pm$1.7 \\ 
		& & \multicolumn{11}{c}{VSRN} \\ 
		{Triplet loss} & {1.5} & {$\alpha=0.2$} &  56.4$\pm$0.7  &  83.6$\pm$0.6 &  90.1$\pm$0.2  & { 76.7$\pm$0.5 } & { 0.63$\pm$0.01 } &  43.1$\pm$0.3  &  74.4$\pm$0.3  &  83.1$\pm$0.4  & { 66.9$\pm$0.3 } &   430.7$\pm$1.8  \\
		{Triplet loss SH} & {1.6} & {$\alpha=0.2$} &  \textbf{68.3}$\pm$1.3  &  \textbf{89.6}$\pm$0.7  &  \textbf{94.0}$\pm$0.5  & { 84.0$\pm$0.5 } &  { 0.73$\pm$0.01 } &  \textbf{51.2}$\pm$0.9  &  \textbf{78.0}$\pm$0.6  &  \textbf{85.6}$\pm$0.5  & { 71.6$\pm$ 0.6 } &  \textbf{466.6}$\pm$3.3  \\
		{NT-Xent} & {1.7} & {$\tau=0.1$} &  50.9 $\pm$0.5 &  78.9$\pm$0.7  &  86.6$\pm$0.4  & { 72.2$\pm$0.4} &  { 0.59$\pm$0.00 } &  40.6$\pm$0.6 &  71.9$\pm$0.2 &  81.7$\pm$0.3  & { 64.7$\pm$0.2 } &  410.6$\pm$1.5  \\
		{SmoothAP} & {1.8} & {$\tau=0.01$} &  63.1$\pm$1.0  &  86.6$\pm$0.8  &  92.4$\pm$0.5  & {  80.7$\pm$0.7  } &  { 0.69$\pm$0.0 } &  45.8$\pm$0.2  &   73.7$\pm$0.3 &  82.3$\pm$0.2  & { 67.3$\pm$0.1 } &  444.0$\pm$2.1  \\ 
			\cmidrule(r){4-13}
		&& \multicolumn{11}{c}{MS-COCO}\textsl{} \\ 
			\cmidrule(r){4-13}
		& & \multicolumn{11}{c}{VSE++} \\ 
		{Triplet loss} & {2.1} & {$\alpha=0.2$} &  22.1$\pm$0.5  &  48.2$\pm$0.3  &  61.7$\pm$0.3  & { 44.0$\pm$0.3 } & { 0.30$\pm$0.00 } & 15.4$\pm$0.1  &  39.5$\pm$0.1  &  53.2$\pm$0.1  & { 36.0$\pm$0.1 }  &  240.0$\pm$0.9  \\
		{Triplet loss SH} & {2.2} & {$\alpha=0.2$} &  \textbf{32.5}$\pm$0.2  &  \textbf{61.6}$\pm$0.3  &  \textbf{73.8}$\pm$0.3  & { 56.0$\pm$0.2 } &  { 0.41$\pm$0.00 } &  \textbf{21.3}$\pm$0.1  &  \textbf{48.1}$\pm$0.1  &  \textbf{61.5}$\pm$0.0  & { 43.6$\pm$0.1 } &  \textbf{298.8}$\pm$0.8  \\
		{NT-Xent} & {2.3} & {$\tau=0.1$} &  25.8$\pm$0.5  &  53.6$\pm$0.5  &  66.1$\pm$0.2  & { 48.5$\pm$0.3 } &  { 0.34$\pm$0.00 } &   18.0$\pm$0.1  &  43.0$\pm$0.1  &  56.6$\pm$0.2 & { 39.2$\pm$0.1} &  263.0$\pm$0.9  \\
		{SmoothAP} & {2.4} & {$\tau=0.01$} &  30.8$\pm$0.3  &  60.3$\pm$0.2  &  \textbf{73.6}$\pm$0.5  & { 54.9$\pm$0.3 } & { 0.40$\pm$0.00 }  &  20.3$\pm$0.2  &  46.5$\pm$0.2  &  60.1$\pm$0.2  & { 42.3$\pm$0.2 } &  291.5$\pm$1.4  \\ 
		& & \multicolumn{11}{c}{VSRN} \\ 
		{Triplet loss} & {2.5} & {$\alpha=0.2$} &  42.9$\pm$0.4  &  74.3$\pm$0.3  &  84.9$\pm$0.4  & { 67.4$\pm$0.3 } &  { 0.52$\pm$0.00 } &  33.5$\pm$0.1  &  65.1$\pm$0.1 &  77.1$\pm$0.2  & { 58.6$\pm$0.1 } &  377.8$\pm$1.2  \\
		{Triplet loss SH} & {2.6} & {$\alpha=0.2$} &  \textbf{48.9}$\pm$0.6  &  \textbf{78.1}$\pm$0.5  &  \textbf{87.4}$\pm$0.2  & { 71.4$\pm$0.4 } &  { 0.57$\pm$0.01 } &  \textbf{37.8}$\pm$0.5  &  \textbf{68.1}$\pm$0.5  &  \textbf{78.9}$\pm$0.3  & { 61.6$\pm$0.4 } &  \textbf{399.0}$\pm$2.3  \\
		{NT-Xent} & {2.7} & {$\tau=0.1$} &  37.9$\pm$0.4  &  69.2$\pm$0.2  &  80.7$\pm$0.3  & { 62.6$\pm$0.1 } &  { 0.47$\pm$0.00 } &  29.5$\pm$0.1  &  61.0$\pm$0.2  &  74.0$\pm$0.2 & { 54.6$\pm$0.1 } &  352.3$\pm$0.5  \\
		{SmoothAP} & {2.8} & {$\tau=0.01$} &  46.0$\pm$0.6  &  76.1$\pm$0.3  &  85.9$\pm$0.3  & { 69.4$\pm$0.3 } &  { 0.54$\pm$0.00 } &  33.8$\pm$0.3  &  64.1$\pm$0.1  &  76.0$\pm$0.24 & { 58.0$\pm$0.2 } &  382.0$\pm$1.1  \\ 
		\bottomrule
	\end{tabular}
}
\end{table*}
